Streaming, Local, and Multi-Level (Hyper)Graph Decomposition

(Hyper)Graph decomposition is a family of problems that aim to break down large (hyper)graphs into smaller sub(hyper)graphs for easier analysis. The importance of this lies in its ability to enable efficient computation on large and complex (hyper)graphs, such as social networks, chemical compounds, and computer networks. This dissertation explores several types of (hyper)graph decomposition problems, including graph partitioning, hypergraph partitioning, local graph clustering, process mapping, and signed graph clustering. Our main focus is on streaming algorithms, local algorithms and multilevel algorithms. In terms of streaming algorithms, we make contributions with highly efficient and effective algorithms for (hyper)graph partitioning and process mapping. In terms of local algorithms, we propose sub-linear algorithms which are effective in detecting high-quality local communities around a given seed node in a graph based on the distribution of a given motif. In terms of multilevel algorithms, we engineer high-quality multilevel algorithms for process mapping and signed graph clustering. We provide a thorough discussion of each algorithm along with experimental results demonstrating their superiority over existing state-of-the-art techniques. The results show that the proposed algorithms achieve improved performance and better solutions in various metrics, making them highly promising for practical applications. Overall, this dissertation showcases the effectiveness of advanced combinatorial algorithmic techniques in solving challenging (hyper)graph decomposition problems.

==> acronyms.tex <==

\usepackage{acro}
\acsetup{first-style=short}

\DeclareAcronym{DNA}{
  short = DNA ,
  long  = Deoxyribonucleic acid ,
}

\DeclareAcronym{RNA}{
  short = RNA ,
  long  = Ribonucleic acid ,
}

\DeclareAcronym{RGEN}{
  short = RGEN ,
  long  = \ac{RNA}-guided endonucleases ,
}

\DeclareAcronym{CRISPR}{
  short = CRISPR ,
  long  = Clustered Regularly Interspaced Short Palindromic Repeats ,
}

\DeclareAcronym{CRISPR-Cas}{
  short = CRISPR-Cas ,
  long  = \ac{CRISPR} associated ,
}

\DeclareAcronym{sgRNA}{
  short = sgRNA ,
  long  = single guide RNA ,
}

==> errors <==
This is pdfTeX, Version 3.141592653-2.6-1.40.24 (TeX Live 2022) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2021-11-15> patch level 1
L3 programming layer <2022-02-24> (./hdphdthesis.cls
Document Class: hdphdthesis 08 Jan 2022 Heidelberg University Dr. rer. nat. The
sis class
(/usr/local/texlive/2022/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/book.cls
Document Class: book 2021/10/04 v1.4n Standard LaTeX document class
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/bk12.clo))
(/usr/local/texlive/2022/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-li
sts.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.c
ode.tex))) (/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/sttools/stfloats.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/emptypage/emptypage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/array.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/lmodern.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/placeins/placeins.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algpseudocode.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algorithmicx.sty
Document Style algorithmicx 1.2 - a greatly improved `algorithmic' style
)
Document Style - pseudocode environments for use with the `algorithmicx' style
) (/usr/local/texlive/2022/texmf-dist/tex/latex/numprint/numprint.sty
No configuration file `numprint.cfg' found.)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2022/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2022/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.
tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothan
dlers.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytopaths.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarypositioning.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/threeparttable/threeparttable.sty
) (/usr/local/texlive/2022/texmf-dist/tex/latex/hvfloat/hvfloat.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/picture/picture.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multido/multido.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/multido/multido.tex
 v1.42, 2010/05/14 <tvz>)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/natbib/natbib.sty

Package natbib Warning: The `cite' package should not be used
(natbib)                with natbib. Use option `sort' instead.

) (/usr/local/texlive/2022/texmf-dist/tex/latex/doi/doi.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.arrows.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.arrows.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarychains.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathreplacing.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduledecoration
s.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathreplacing.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/framed/framed.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xifthen/xifthen.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense-english.ldf
)) (/usr/local/texlive/2022/texmf-dist/tex/latex/ccicons/ccicons.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmr.fd)

LaTeX Warning: Unused global option(s):
    [mathcomp,marginleft,marginright,margintop,marginbottom,bindingoffset].

No file main.aux.
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/ltcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2022/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omllmm.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmsy.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omxlmex.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msb.cfg) [1.1{/usr/l
ocal/texlive/2022/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2.2] [3.3]
[4.4] (./chapters/abstracts.tex [5.5] [6.6]
Underfull \hbox (badness 5696) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Dis-ser-ta-tion be-fasst sich mit der Un-ter-suchung ver-
schiedener Arten von

Underfull \hbox (badness 6708) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Multi-Level-Algorithmen. Im Bere-ich der Streaming-Algori
thmen leis-ten

Underfull \hbox (badness 10000) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) wir Beitr^^?age mit hochef-fizien-ten und ef-fek-tiven Al
-go-rith-men f^^?ur die
[7.7]) (./chapters/acknowledgements.tex [8.8]
Underfull \vbox (badness 1533) has occurred while \output is active [9.9]
Underfull \vbox (badness 1515) has occurred while \output is active [10.10]
[11.11]) (./chapters/publications.tex [12.12]
Underfull \hbox (badness 10000) in paragraph at lines 2--3

[13.13] [14.14] [15.15]) [16.16] [17.17] [18.18] (./chapters/introduction.tex
Chapter 1.

Package natbib Warning: Citation `Garey1974' on page 1 undefined on input line 
32.


Package natbib Warning: Citation `BuiJ92' on page 1 undefined on input line 32.



Package natbib Warning: Citation `tsourakakis2014fennel' on page 1 undefined on
 input line 34.


Package natbib Warning: Citation `awadelkarim2020prioritized' on page 1 undefin
ed on input line 34.


Package natbib Warning: Citation `jafari2021fast' on page 1 undefined on input 
line 34.


Package natbib Warning: Citation `mayer2018adwise' on page 1 undefined on input
 line 34.


Package natbib Warning: Citation `hoang2019cusp' on page 1 undefined on input l
ine 34.


Package natbib Warning: Citation `alistarh2015streaming' on page 1 undefined on
 input line 34.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 1 undefined o
n input line 34.


Package natbib Warning: Citation `HeiStream' on page 1 undefined on input line 
34.


Package natbib Warning: Citation `StreamMultiSection' on page 1 undefined on in
put line 34.


Package natbib Warning: Citation `freight_paper' on page 1 undefined on input l
ine 34.

[1.19]

Package natbib Warning: Citation `kannan2004clusterings' on page 2 undefined on
 input line 49.


Package natbib Warning: Citation `epasto2014reduce' on page 2 undefined on inpu
t line 51.


Package natbib Warning: Citation `jeub2015think' on page 2 undefined on input l
ine 51.


Package natbib Warning: Citation `voevodski2009spectral' on page 2 undefined on
 input line 51.


Package natbib Warning: Citation `wagner1993between' on page 2 undefined on inp
ut line 52.


Package natbib Warning: Citation `andersen2006local' on page 2 undefined on inp
ut line 54.


Package natbib Warning: Citation `leskovec2009community' on page 2 undefined on
 input line 54.


Package natbib Warning: Citation `chung2013solving' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `li2015uncovering' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `fountoulakis2020flowbased' on page 2 undefine
d on input line 54.


Package natbib Warning: Citation `yin2017local' on page 2 undefined on input li
ne 54.


Package natbib Warning: Citation `zhang2019local' on page 2 undefined on input 
line 54.


Package natbib Warning: Citation `meng2019local' on page 2 undefined on input l
ine 54.


Package natbib Warning: Citation `murali2020online' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `yin2017local' on page 2 undefined on input li
ne 55.


Underfull \vbox (badness 10000) has occurred while \output is active [2.20]

Package natbib Warning: Citation `kannan2004clusterings' on page 3 undefined on
 input line 63.


Package natbib Warning: Citation `brandes2007modularity' on page 3 undefined on
 input line 63.


Package natbib Warning: Citation `application_review' on page 3 undefined on in
put line 69.


Package natbib Warning: Citation `DBLP:phd/dnb/Wakabayashi86' on page 3 undefin
ed on input line 70.

[3.21] [4.22] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmss.fd)

Package natbib Warning: Citation `mqipaper2004' on page 5 undefined on input li
ne 133.

[5.23]

LaTeX Warning: Reference `chap:Preliminaries' on page 6 undefined on input line
 172.


LaTeX Warning: Reference `chap:Related Work' on page 6 undefined on input line 
173.


LaTeX Warning: Reference `chap:Streaming Algorithms' on page 6 undefined on inp
ut line 174.


LaTeX Warning: Reference `chap:Local Algorithms' on page 6 undefined on input l
ine 174.


LaTeX Warning: Reference `chap:Multilevel Algorithms' on page 6 undefined on in
put line 174.


LaTeX Warning: Reference `chap:Discussion' on page 6 undefined on input line 17
5.

[6.24]) [7.25] (./chapters/preliminaries.tex [8.26]
Chapter 2.
[9.27]

Package natbib Warning: Citation `brandes2007modularity' on page 10 undefined o
n input line 78.


Package natbib Warning: Citation `kannan2004clusterings' on page 10 undefined o
n input line 78.


Package natbib Warning: Citation `benson2016higher' on page 10 undefined on inp
ut line 82.

[10.28]

Package natbib Warning: Citation `brandfass2013rank' on page 11 undefined on in
put line 105.

[11.29]

LaTeX Warning: Reference `eq:process_mapping_obj' on page 12 undefined on input
 line 117.


Package natbib Warning: Citation `ford_fulkerson_1956' on page 12 undefined on 
input line 143.

[12.30]

Package natbib Warning: Citation `push_relabel88' on page 13 undefined on input
 line 149.


Package natbib Warning: Citation `veldt2022hypergraph' on page 13 undefined on 
input line 155.


Package natbib Warning: Citation `lawler1973cutsets' on page 13 undefined on in
put line 155.


LaTeX Warning: Reference `fig:social_hyperedge_expansion' on page 13 undefined 
on input line 163.


LaTeX Warning: Reference `fig:sgc_clustercontraction' on page 13 undefined on i
nput line 182.


Underfull \vbox (badness 10000) has occurred while \output is active [13.31]

LaTeX Warning: Reference `fig:sgc_localsearch' on page 14 undefined on input li
ne 195.

[14.32 <./chapters/social/HyperEdgeExpansions.png (PNG copy)>]

Package natbib Warning: Citation `kaffpa' on page 15 undefined on input line 20
0.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 15 undefi
ned on input line 213.


Package natbib Warning: Citation `evolutionary_book' on page 15 undefined on in
put line 230.


Package natbib Warning: Citation `sastry2014genetic' on page 15 undefined on in
put line 231.


Package natbib Warning: Citation `goldberg1989messy' on page 15 undefined on in
put line 233.


Package natbib Warning: Citation `Michalewicz:1996:GAD:229930' on page 15 undef
ined on input line 234.

[15.33 <./chapters/heistream/pics/MGP.png (PNG copy)> <./chapters/SignedCluster
EvolutionaryPaper/pics/cluster_contraction.png (PNG copy)>]

LaTeX Warning: Reference `fig:streaming' on page 16 undefined on input line 244
.


Underfull \vbox (badness 10000) has occurred while \output is active [16.34 <./
chapters/SignedClusterEvolutionaryPaper/pics/LP_illustration.png (PNG copy)>]

Package natbib Warning: Citation `snapnets' on page 17 undefined on input line 
287.


Package natbib Warning: Citation `nr-aaai15' on page 17 undefined on input line
 287.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 287.


Package natbib Warning: Citation `kappa' on page 17 undefined on input line 287
.


Package natbib Warning: Citation `funke2019communication' on page 17 undefined 
on input line 287.


Package natbib Warning: Citation `snapnets' on page 17 undefined on input line 
289.


Package natbib Warning: Citation `nr-aaai15' on page 17 undefined on input line
 289.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 290.


Package natbib Warning: Citation `kappa' on page 17 undefined on input line 294
.


Package natbib Warning: Citation `funke2019communication' on page 17 undefined 
on input line 295.


Package natbib Warning: Citation `DBLP:journals/corr/abs-2003-00736' on page 17
 undefined on input line 295.


LaTeX Warning: Reference `tab:heistream_graphs' on page 17 undefined on input l
ine 296.


Package natbib Warning: Citation `soper2004combined' on page 17 undefined on in
put line 388.


Package natbib Warning: Citation `davis2011university' on page 17 undefined on 
input line 389.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 390.


Package natbib Warning: Citation `DSSW09' on page 17 undefined on input line 39
3.


LaTeX Warning: Reference `tab:test_instances_walshaw' on page 17 undefined on i
nput line 394.

[17.35 <./chapters/more_recent_partitioning_survey/img/streaming/streaming.png 
(PNG copy)>]

Package natbib Warning: Citation `snapnets' on page 18 undefined on input line 
505.


Package natbib Warning: Citation `nr-aaai15' on page 18 undefined on input line
 505.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 18 und
efined on input line 505.


LaTeX Warning: Reference `tab:lmcvhgp_graphs' on page 18 undefined on input lin
e 507.


Package natbib Warning: Citation `yin2017local' on page 18 undefined on input l
ine 509.

[18.36]

Package natbib Warning: Citation `schlag2016k' on page 19 undefined on input li
ne 520.


Package natbib Warning: Citation `alpert1998ispd98' on page 19 undefined on inp
ut line 522.


Package natbib Warning: Citation `davis2011university' on page 19 undefined on 
input line 523.


Package natbib Warning: Citation `Belov2014' on page 19 undefined on input line
 524.


LaTeX Warning: Reference `tab:sgc_graphs' on page 19 undefined on input line 53
3.


Package natbib Warning: Citation `snap' on page 19 undefined on input line 534.



Package natbib Warning: Citation `konect' on page 19 undefined on input line 53
4.


Underfull \vbox (badness 10000) has occurred while \output is active [19.37]
[20.38] [21.39 <./chapters/social/plots/mqi_clique/tim/pp_chart.png (PNG copy)>
]

LaTeX Warning: Reference `fig:prel_SIMPLEstateoftheart_graph_pp' on page 22 und
efined on input line 613.

) [22.40] (./chapters/related_work.tex
Chapter 3.

Package natbib Warning: Citation `ccatalyurek2011patoh' on page 23 undefined on
 input line 13.


Package natbib Warning: Citation `parmetis-conference' on page 23 undefined on 
input line 13.


Package natbib Warning: Citation `hMetis' on page 23 undefined on input line 13
.


Package natbib Warning: Citation `Pellegrini96experimentalanalysis' on page 23 
undefined on input line 13.


Package natbib Warning: Citation `HYPE2018' on page 23 undefined on input line 
13.


Package natbib Warning: Citation `kabapeE' on page 23 undefined on input line 1
3.


Package natbib Warning: Citation `gottesburen2021deep' on page 23 undefined on 
input line 13.


Package natbib Warning: Citation `schlag2016k' on page 23 undefined on input li
ne 13.


Package natbib Warning: Citation `mt-kahypar-d' on page 23 undefined on input l
ine 13.


Package natbib Warning: Citation `DBLP:conf/europar/Akhremtsev0018' on page 23 
undefined on input line 13.


Package natbib Warning: Citation `more_recent_advances_hgp' on page 23 undefine
d on input line 14.


Package natbib Warning: Citation `SPPGPOverviewPaper' on page 23 undefined on i
nput line 14.


Package natbib Warning: Citation `DBLP:reference/bdt/0003S19' on page 23 undefi
ned on input line 14.


Package natbib Warning: Citation `stanton2012streaming' on page 23 undefined on
 input line 26.

[23.41]

Package natbib Warning: Citation `stanton2014streaming' on page 24 undefined on
 input line 38.


Package natbib Warning: Citation `chung2003generalizations' on page 24 undefine
d on input line 40.


Package natbib Warning: Citation `tsourakakis2014fennel' on page 24 undefined o
n input line 42.


Package natbib Warning: Citation `brandes2007modularity' on page 24 undefined o
n input line 43.


Package natbib Warning: Citation `stanton2012streaming' on page 24 undefined on
 input line 49.


Package natbib Warning: Citation `zhang2018akin' on page 24 undefined on input 
line 54.


Package natbib Warning: Citation `hamers1989similarity' on page 24 undefined on
 input line 57.


Package natbib Warning: Citation `nishimura2013restreaming' on page 24 undefine
d on input line 73.


Package natbib Warning: Citation `stanton2012streaming' on page 24 undefined on
 input line 77.


Package natbib Warning: Citation `tsourakakis2014fennel' on page 24 undefined o
n input line 77.

[24.42]

Package natbib Warning: Citation `awadelkarim2020prioritized' on page 25 undefi
ned on input line 86.


Package natbib Warning: Citation `patwary2019window' on page 25 undefined on in
put line 97.


Package natbib Warning: Citation `jafari2021fast' on page 25 undefined on input
 line 102.

[25.43]

Package natbib Warning: Citation `alistarh2015streaming' on page 26 undefined o
n input line 119.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 26 undefined 
on input line 128.


Package natbib Warning: Citation `alistarh2015streaming' on page 26 undefined o
n input line 128.

[26.44]

Package natbib Warning: Citation `benson2015tensor' on page 27 undefined on inp
ut line 201.


Package natbib Warning: Citation `yin2017local' on page 27 undefined on input l
ine 201.


Package natbib Warning: Citation `klymko2014using' on page 27 undefined on inpu
t line 201.


Package natbib Warning: Citation `prvzulj2007biological' on page 27 undefined o
n input line 201.


Package natbib Warning: Citation `tsourakakis2017scalable' on page 27 undefined
 on input line 201.


Package natbib Warning: Citation `kloster2014heat' on page 27 undefined on inpu
t line 203.


Package natbib Warning: Citation `li2015uncovering' on page 27 undefined on inp
ut line 203.


Package natbib Warning: Citation `mahoney2012local' on page 27 undefined on inp
ut line 203.


Package natbib Warning: Citation `cui2014local' on page 27 undefined on input l
ine 203.


Package natbib Warning: Citation `sozio2010community' on page 27 undefined on i
nput line 203.

[27.45]

Package natbib Warning: Citation `rohe2013blessing' on page 28 undefined on inp
ut line 210.


Package natbib Warning: Citation `huang2014querying' on page 28 undefined on in
put line 213.


Package natbib Warning: Citation `cohen2008trusses' on page 28 undefined on inp
ut line 213.


Package natbib Warning: Citation `yin2017local' on page 28 undefined on input l
ine 217.


Package natbib Warning: Citation `zhang2019local' on page 28 undefined on input
 line 224.


Package natbib Warning: Citation `meng2019local' on page 28 undefined on input 
line 231.


Underfull \vbox (badness 3657) has occurred while \output is active [28.46]

Package natbib Warning: Citation `zhou2021high' on page 29 undefined on input l
ine 238.


Package natbib Warning: Citation `spielman2013local' on page 29 undefined on in
put line 241.


Package natbib Warning: Citation `shang2022local' on page 29 undefined on input
 line 245.


Package natbib Warning: Citation `DBLP:journals/fgcs/WalshawC01' on page 29 und
efined on input line 267.


Package natbib Warning: Citation `DBLP:conf/hpcn/PellegriniR96' on page 29 unde
fined on input line 267.


Package natbib Warning: Citation `schulz2017better' on page 29 undefined on inp
ut line 268.


Package natbib Warning: Citation `brandfass2013rank' on page 29 undefined on in
put line 268.


Package natbib Warning: Citation `heider1972computationally' on page 29 undefin
ed on input line 268.


Package natbib Warning: Citation `muller2013optimale' on page 29 undefined on i
nput line 268.


Package natbib Warning: Citation `glantz2015algorithms' on page 29 undefined on
 input line 268.


LaTeX Warning: Reference `eq:process_mapping_obj' on page 29 undefined on input
 line 270.


Package natbib Warning: Citation `GPOverviewBook' on page 29 undefined on input
 line 274.


Package natbib Warning: Citation `SPPGPOverviewPaper' on page 29 undefined on i
nput line 274.

[29.47]

Package natbib Warning: Citation `muller2013optimale' on page 30 undefined on i
nput line 289.


Package natbib Warning: Citation `heider1972computationally' on page 30 undefin
ed on input line 294.


Package natbib Warning: Citation `brandfass2013rank' on page 30 undefined on in
put line 299.


Package natbib Warning: Citation `DBLP:conf/ipps/DeveciKUC15' on page 30 undefi
ned on input line 304.


Package natbib Warning: Citation `Scotch' on page 30 undefined on input line 31
0.


Package natbib Warning: Citation `Walshaw07' on page 30 undefined on input line
 310.


Package natbib Warning: Citation `8666156' on page 30 undefined on input line 3
14.


Package natbib Warning: Citation `DBLP:journals/tpds/DeveciRDC16' on page 30 un
defined on input line 316.


Underfull \vbox (badness 1515) has occurred while \output is active [30.48]

Package natbib Warning: Citation `vogelstein2015fast' on page 31 undefined on i
nput line 322.


Package natbib Warning: Citation `umeyama1988eigendecomposition' on page 31 und
efined on input line 326.


Package natbib Warning: Citation `singh2007pairwise' on page 31 undefined on in
put line 326.


Package natbib Warning: Citation `zaslavskiy2008path' on page 31 undefined on i
nput line 326.


Package natbib Warning: Citation `burkard1997qaplib' on page 31 undefined on in
put line 326.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 331.


Package natbib Warning: Citation `muller2013optimale' on page 31 undefined on i
nput line 334.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 335.


Package natbib Warning: Citation `glantz2018topology' on page 31 undefined on i
nput line 338.


Package natbib Warning: Citation `Scotch' on page 31 undefined on input line 34
2.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 342.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 349.


Package natbib Warning: Citation `kaHIPHomePage' on page 31 undefined on input 
line 350.


Package natbib Warning: Citation `brandfass2013rank' on page 31 undefined on in
put line 353.


Package natbib Warning: Citation `muller2013optimale' on page 31 undefined on i
nput line 355.


Package natbib Warning: Citation `Walshaw07' on page 31 undefined on input line
 355.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 355.


Package natbib Warning: Citation `GlobalMultisection' on page 31 undefined on i
nput line 356.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 356.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 358.


Underfull \vbox (badness 1515) has occurred while \output is active [31.49]

Package natbib Warning: Citation `PredariProcessMapping21' on page 32 undefined
 on input line 366.


Package natbib Warning: Citation `parmetis-conference' on page 32 undefined on 
input line 370.


Package natbib Warning: Citation `DBLP:journals/tpds/MeyerhenkeSS17' on page 32
 undefined on input line 370.


Package natbib Warning: Citation `von2020efficient' on page 32 undefined on inp
ut line 377.


Package natbib Warning: Citation `viemaWebsite' on page 32 undefined on input l
ine 384.


Package natbib Warning: Citation `yang2007community' on page 32 undefined on in
put line 400.


Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 32 unde
fined on input line 400.


Package natbib Warning: Citation `traag2009community' on page 32 undefined on i
nput line 400.


Package natbib Warning: Citation `correlationclustering_overall' on page 32 und
efined on input line 400.


Package natbib Warning: Citation `demaine2006correlation' on page 32 undefined 
on input line 400.


Package natbib Warning: Citation `grotschel1989cutting' on page 32 undefined on
 input line 400.


Package natbib Warning: Citation `dinh2015toward' on page 32 undefined on input
 line 400.


Package natbib Warning: Citation `miyauchi2015redundant' on page 32 undefined o
n input line 400.


Package natbib Warning: Citation `miyauchi2018exact' on page 32 undefined on in
put line 400.


Package natbib Warning: Citation `kunegis2010spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `gallier2016spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `knyazev2018spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `mercado2019spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `he2011ant' on page 32 undefined on input line
 401.


Package natbib Warning: Citation `zhu2018novel' on page 32 undefined on input l
ine 401.


Package natbib Warning: Citation `brusco2019partitioning' on page 32 undefined 
on input line 401.


Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 32 unde
fined on input line 401.


Package natbib Warning: Citation `abdulrahman2020enhanced' on page 32 undefined
 on input line 401.


Package natbib Warning: Citation `chen2022iterated' on page 32 undefined on inp
ut line 401.


Package natbib Warning: Citation `gallier2016spectral' on page 32 undefined on 
input line 402.


Package natbib Warning: Citation `surveyTangCAL16' on page 32 undefined on inpu
t line 402.


Package natbib Warning: Citation `tomasso2021advances' on page 32 undefined on 
input line 402.

[32.50]

Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 429.


Package natbib Warning: Citation `bailoni2019generalized' on page 33 undefined 
on input line 431.


Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 432.


Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 440.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 33 undefined on in
put line 444.

[33.51]

Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 34 unde
fined on input line 454.


Package natbib Warning: Citation `gomez2009analysis' on page 34 undefined on in
put line 455.


Underfull \vbox (badness 10000) has occurred while \output is active [34.52]

Package natbib Warning: Citation `grotschel1989cutting' on page 35 undefined on
 input line 471.


Package natbib Warning: Citation `dinh2015toward' on page 35 undefined on input
 line 473.


Package natbib Warning: Citation `grotschel1989cutting' on page 35 undefined on
 input line 473.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 473.


Package natbib Warning: Citation `dinh2015toward' on page 35 undefined on input
 line 473.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 474.


Package natbib Warning: Citation `miyauchi2018exact' on page 35 undefined on in
put line 476.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 476.


Package natbib Warning: Citation `koshimura2022concise' on page 35 undefined on
 input line 478.


Package natbib Warning: Citation `miyauchi2018exact' on page 35 undefined on in
put line 478.

[35.53]) [36.54] (./chapters/chapter1.tex
Chapter 4.

Package natbib Warning: Citation `HeiStream' on page 37 undefined on input line
 17.


Package natbib Warning: Citation `StreamMultiSection' on page 37 undefined on i
nput line 17.


Package natbib Warning: Citation `freight_paper' on page 37 undefined on input 
line 17.

(./chapters/heistream/chapter.tex
Underfull \vbox (badness 10000) has occurred while \output is active [37.55]

LaTeX Warning: Reference `alg:heistream_overall_algorithm' on page 38 undefined
 on input line 186.


LaTeX Warning: Reference `fig:heistream_comprehensive_scheme' on page 38 undefi
ned on input line 186.

[38.56]

LaTeX Warning: Reference `fig:heistream_comprehensive_scheme' on page 39 undefi
ned on input line 237.


Underfull \vbox (badness 10000) has occurred while \output is active [39.57 <./
chapters/heistream/MultilevelBufferedStreamGP.png (PNG copy)>]

LaTeX Warning: Reference `fig:sgc_MSGC' on page 40 undefined on input line 246.



Package natbib Warning: Citation `tsourakakis2014fennel' on page 40 undefined o
n input line 251.

[40.58]

LaTeX Warning: Reference `eq:gen_fennel' on page 41 undefined on input line 265
.


LaTeX Warning: Reference `theo:generalized_fennel' on page 41 undefined on inpu
t line 268.


LaTeX Warning: Reference `eq:gain_w' on page 41 undefined on input line 292.


LaTeX Warning: Reference `eq:gain_S' on page 41 undefined on input line 292.


LaTeX Warning: Reference `eq:equality1' on page 41 undefined on input line 292.



LaTeX Warning: Reference `eq:equality2' on page 41 undefined on input line 292.



LaTeX Warning: Reference `eq:equality1' on page 41 undefined on input line 301.



LaTeX Warning: Reference `eq:equality2' on page 41 undefined on input line 301.


[41.59]

Package natbib Warning: Citation `kaffpa' on page 42 undefined on input line 30
7.


Package natbib Warning: Citation `karypis1998fast' on page 42 undefined on inpu
t line 308.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 42 undefi
ned on input line 316.


LaTeX Warning: Reference `fig:sgc_clustercontraction' on page 42 undefined on i
nput line 317.


Package natbib Warning: Citation `labelpropagationclustering' on page 42 undefi
ned on input line 324.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 42 undefi
ned on input line 324.

[42.60]

LaTeX Warning: Reference `eq:gen_fennel' on page 43 undefined on input line 360
.


Underfull \vbox (badness 10000) has occurred while \output is active [43.61]
[44.62]

Package natbib Warning: Citation `jafari2021fast' on page 45 undefined on input
 line 433.


Package natbib Warning: Citation `jafari2021fast' on page 45 undefined on input
 line 435.


LaTeX Warning: Reference `tab:heistream_graphs' on page 45 undefined on input l
ine 442.

[45.63]

LaTeX Warning: Reference `tab:heistream_graphs' on page 46 undefined on input l
ine 559.


LaTeX Warning: Reference `fig:heistream_res_rep_label' on page 46 undefined on 
input line 563.


LaTeX Warning: Reference `fig:heistream_tim_rep_label' on page 46 undefined on 
input line 563.


LaTeX Warning: Reference `fig:heistream_StopRule' on page 46 undefined on input
 line 581.


LaTeX Warning: Reference `fig:heistream_StopRule' on page 46 undefined on input
 line 583.


LaTeX Warning: Reference `tab:heistream_graphs' on page 46 undefined on input l
ine 602.


LaTeX Warning: Reference `fig:heistream_res_batch_noFennel' on page 46 undefine
d on input line 603.


LaTeX Warning: Reference `fig:heistream_tim_batch_noFennel' on page 46 undefine
d on input line 603.

[46.64] [47.65 <./chapters/heistream/Images/repetitions_label_prop/res_rep_labe
l.png (PNG copy)> <./chapters/heistream/Images/tim_TIMErep_label/tim_TIMErep_la
bel.png (PNG copy)> <./chapters/heistream/Images/StopRule/res_StopRule.png (PNG
 copy)> <./chapters/heistream/Images/restream/res_restream.png (PNG copy)> <./c
hapters/heistream/Images/batch_noFennel/res_batch_noFennel.png (PNG copy)> <./c
hapters/heistream/Images/tim_TIMEbatch_noFennel/tim_TIMEbatch_noFennel.png (PNG
 copy)>]

LaTeX Warning: Reference `fig:heistream_res_ghost' on page 48 undefined on inpu
t line 616.


LaTeX Warning: Reference `fig:heistream_tim_ghost' on page 48 undefined on inpu
t line 616.


LaTeX Warning: Reference `fig:heistream_res_restream' on page 48 undefined on i
nput line 630.


Underfull \vbox (badness 1348) has occurred while \output is active [48.66 <./c
hapters/heistream/Images/ghost/res_ghost.png (PNG copy)> <./chapters/heistream/
Images/tim_TIMEghost/tim_TIMEghost.png (PNG copy)>]
Overfull \hbox (11.6059pt too wide) in paragraph at lines 665--701
 [][] 

LaTeX Warning: Reference `tab:heistream_graphs' on page 49 undefined on input l
ine 770.

[49.67 <./chapters/heistream/Images/MultiLDG/comparison_MultiLDG_vertical/Multi
LDGFullBuffer.png (PNG copy)>] [50.68]

Package natbib Warning: Citation `karypis1998fast' on page 51 undefined on inpu
t line 778.


Package natbib Warning: Citation `kaffpa' on page 51 undefined on input line 77
8.


LaTeX Warning: Reference `tab:heistream_multiLDG' on page 51 undefined on input
 line 790.

[51.69 <./chapters/heistream/Images/res_stateOfTheArtPlots/res_stateOfTheArtPlo
ts.png (PNG copy)> <./chapters/heistream/Images/tim_stateOfTheArtPlots/tim_stat
eOfTheArtPlots.png (PNG copy)> <./chapters/heistream/Images/res_stateOfTheArtPl
ots/pp_res_stateOfTheArtPlots.png (PNG copy)> <./chapters/heistream/Images/tim_
stateOfTheArtPlots/pp_tim_stateOfTheArtPlots.png (PNG copy)>]

LaTeX Warning: Reference `fig:heistream_multiLDG' on page 52 undefined on input
 line 797.


Package natbib Warning: Citation `jafari2021fast' on page 52 undefined on input
 line 798.


LaTeX Warning: Reference `fig:heistream_res_InitFennelOpt4' on page 52 undefine
d on input line 804.


LaTeX Warning: Reference `fig:heistream_tim_InitFennelOpt4' on page 52 undefine
d on input line 804.


LaTeX Warning: Reference `fig:heistream_pp_res_InitFennelOpt4' on page 52 undef
ined on input line 805.


LaTeX Warning: Reference `fig:heistream_pp_tim_InitFennelOpt4' on page 52 undef
ined on input line 805.


Underfull \vbox (badness 5939) has occurred while \output is active [52.70 <./c
hapters/heistream/Images/res_restreamStateOfTheArtPlots/pp_res_restreamStateOfT
heArtPlots.png (PNG copy)>]

LaTeX Warning: Reference `tab:heistream_multiLDG' on page 53 undefined on input
 line 826.


LaTeX Warning: Reference `fig:heistream_restream' on page 53 undefined on input
 line 827.


LaTeX Warning: Reference `fig:heistream_visualization' on page 53 undefined on 
input line 845.

[53.71] [54.72 <./chapters/heistream/Visualization.png (PNG copy)>]
Overfull \hbox (0.9859pt too wide) in paragraph at lines 867--940
 [][] 

LaTeX Warning: Float too large for page by 23.98486pt on input line 942.


LaTeX Warning: Reference `tab:heistream_graphs' on page 55 undefined on input l
ine 947.


LaTeX Warning: Reference `tab:heistream_hugeResults' on page 55 undefined on in
put line 952.


LaTeX Warning: Reference `tab:heistream_hugeResults' on page 55 undefined on in
put line 953.


LaTeX Warning: Reference `tab:heistream_graphs' on page 55 undefined on input l
ine 954.

[55.73] [56.74]) (./chapters/recmultisec/chapter.tex

Package natbib Warning: Citation `schulz2017better' on page 57 undefined on inp
ut line 124.


Package natbib Warning: Citation `GlobalMultisection' on page 57 undefined on i
nput line 124.


Package natbib Warning: Citation `GlobalMultisection' on page 57 undefined on i
nput line 131.

[57.75]

LaTeX Warning: Reference `alg:recmultisec_One-pass Process Mapping' on page 58 
undefined on input line 141.


LaTeX Warning: Reference `fig:recmultisec_hierarchy_problems' on page 58 undefi
ned on input line 141.


LaTeX Warning: Reference `subsec:recmultisec_subproblems' on page 58 undefined 
on input line 141.


Underfull \vbox (badness 2012) has occurred while \output is active [58.76]

LaTeX Warning: Reference `theo:recmultisec_num_blocks_msec' on page 59 undefine
d on input line 204.

[59.77 <./chapters/recmultisec/Multi-Section.png (PNG copy)>]

LaTeX Warning: Reference `theo:recmultisec_running_time_msec' on page 60 undefi
ned on input line 220.

[60.78]

Package natbib Warning: Citation `more_recent_advances_hgp' on page 61 undefine
d on input line 298.


LaTeX Warning: Reference `alg:recmultisec_Recursively Define Subproblems' on pa
ge 61 undefined on input line 304.


LaTeX Warning: Reference `alg:recmultisec_Recursively Define Subproblems' on pa
ge 61 undefined on input line 332.


LaTeX Warning: Reference `alg:recmultisec_One-pass Process Mapping' on page 61 
undefined on input line 334.


LaTeX Warning: Reference `theo:recmultisec_mem_usage_msec' on page 61 undefined
 on input line 335.


LaTeX Warning: Reference `theo:recmultisec_expected_running_time_bisec' on page
 61 undefined on input line 336.

[61.79]

LaTeX Warning: Reference `alg:recmultisec_Recursively Define Subproblems' on pa
ge 62 undefined on input line 370.

[62.80]

LaTeX Warning: Reference `alg:recmultisec_One-pass Process Mapping' on page 63 
undefined on input line 403.


Underfull \vbox (badness 10000) has occurred while \output is active [63.81]

Package natbib Warning: Citation `tsourakakis2014fennel' on page 64 undefined o
n input line 431.


LaTeX Warning: Reference `chap:intmap_Multilevel Process Mapping' on page 64 un
defined on input line 435.


Package natbib Warning: Citation `gottesburen2021deep' on page 64 undefined on 
input line 436.


LaTeX Warning: Reference `tab:heistream_graphs' on page 64 undefined on input l
ine 446.


Package natbib Warning: Citation `schulz2017better' on page 64 undefined on inp
ut line 449.


Package natbib Warning: Citation `GlobalMultisection' on page 64 undefined on i
nput line 449.

[64.82]

LaTeX Warning: Reference `eq:process_mapping_obj' on page 65 undefined on input
 line 458.


LaTeX Warning: Reference `tab:heistream_graphs' on page 65 undefined on input l
ine 777.


Overfull \hbox (0.77881pt too wide) in paragraph at lines 798--799
\OT1/lmr/m/n/12 (-20) In this sec-tion, we show ex-per-i-ments in which we com-
pare $[]$

LaTeX Warning: Reference `fig:recmultisec_stateoftheartMap_res' on page 65 unde
fined on input line 804.


LaTeX Warning: Reference `fig:recmultisec_stateoftheartMap_respp' on page 65 un
defined on input line 811.

[65.83] [66.84 <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/chart
.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/pp_
chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/re
s/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/
tim/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateofthear
tPar/GP/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoft
heartPar/tim/chart.png (PNG copy)>] [67.85 <./chapters/recmultisec/Images/tunin
g/parallelSpeedups/speedup/soc-orkut-dir/chart.png (PNG copy)> <./chapters/recm
ultisec/Images/tuning/parallelSpeedups/times/soc-orkut-dir/chart.png (PNG copy)
> <./chapters/recmultisec/Images/tuning/parallelSpeedups/speedup/HV15R/chart.pn
g (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/times/HV15
R/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/
speedup/soc-LiveJournal1/chart.png (PNG copy)> <./chapters/recmultisec/Images/t
uning/parallelSpeedups/times/soc-LiveJournal1/chart.png (PNG copy)>]

LaTeX Warning: Reference `fig:recmultisec_stateoftheartPar_res' on page 68 unde
fined on input line 818.


LaTeX Warning: Reference `fig:recmultisec_stateoftheartPar_GPpp' on page 68 und
efined on input line 823.


LaTeX Warning: Reference `fig:recmultisec_stateoftheartPar_tim' on page 68 unde
fined on input line 830.


LaTeX Warning: Reference `fig:recmultisec_stateoftheartPar_timpp' on page 68 un
defined on input line 836.


LaTeX Warning: Reference `theo:recmultisec_expected_running_time_bisec' on page
 68 undefined on input line 837.


LaTeX Warning: Reference `subsec:recmultisec_State-of-the-Art' on page 68 undef
ined on input line 886.

[68.86]

LaTeX Warning: Reference `fig:recmultisec_state-of_the_art_parallel' on page 69
 undefined on input line 892.


LaTeX Warning: Reference `tab:recmultisec_scalability' on page 69 undefined on 
input line 893.


Package natbib Warning: Citation `gottesburen2021deep' on page 69 undefined on 
input line 900.

) (./chapters/freight/chapter.tex [69.87]

LaTeX Warning: Reference `eq:freight_FREIGHT' on page 70 undefined on input lin
e 172.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 70 undefined on input lin
e 174.

[70.88]
Overfull \hbox (10.08015pt too wide) in paragraph at lines 181--185
\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m/it/12 V[]\OT1/lmr/m/n/12 (-
20) )[]$, where the weight $\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m
/it/12 v\OT1/lmr/m/n/12 (-20) )$ of $\OML/lmm/m/it/12 v$ \OT1/lmr/m/n/12 (-20) 
is []. 

LaTeX Warning: Reference `fig:freight_StreamingModel' on page 71 undefined on i
nput line 205.


Package natbib Warning: Citation `alistarh2015streaming' on page 71 undefined o
n input line 209.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 71 undefined 
on input line 209.

[71.89 <./chapters/freight/streaming.png (PNG copy)>]

LaTeX Warning: Reference `eq:freight_FREIGHT' on page 72 undefined on input lin
e 218.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 72 undefined on input lin
e 226.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 226.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 72 undefined on input
 line 226.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 72 undefined on input lin
e 227.


LaTeX Warning: Reference `fig:freight_DecomposeEquation' on page 72 undefined o
n input line 228.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 72 undefined on input lin
e 247.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 247.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 72 undefined on input
 line 247.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 72 undefined on input lin
e 247.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 254.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 72 undefined on input
 line 254.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 255.


LaTeX Warning: Reference `theo:freight_E_1' on page 72 undefined on input line 
255.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 72 undefined on input
 line 256.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 72 undefined on input
 line 257.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 261.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 266.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 72 undefined on input
 line 267.

[72.90]

LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 73 und
efined on input line 288.


LaTeX Warning: Reference `fig:freight_SortingArray' on page 73 undefined on inp
ut line 288.


LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 73 und
efined on input line 289.


LaTeX Warning: Reference `fig:freight_SortingArray' on page 73 undefined on inp
ut line 297.


LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 73 und
efined on input line 297.


LaTeX Warning: Reference `theo:freight_sorting_correctness' on page 73 undefine
d on input line 298.


LaTeX Warning: Reference `theo:freight_E_2' on page 73 undefined on input line 
299.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 73 undefined on input
 line 299.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 73 undefined on input
 line 299.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 73 undefined on input lin
e 299.


LaTeX Warning: Reference `theo:freight_E_1' on page 73 undefined on input line 
302.


LaTeX Warning: Reference `theo:freight_E_2' on page 73 undefined on input line 
302.


LaTeX Warning: Reference `cor:freight_complexity_without_sampling' on page 73 u
ndefined on input line 302.


Underfull \vbox (badness 1694) has occurred while \output is active [73.91 <./c
hapters/freight/DecomposeEqFREIGHT.png (PNG copy)>]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `htbp') on input line 305.


LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 74 und
efined on input line 336.

[74.92 <./chapters/freight/SortingArrays.png (PNG copy)>]

LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 75 undefined on input
 line 349.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 75 undefined on input
 line 349.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 75 undefined on input lin
e 349.


LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 75 und
efined on input line 354.


LaTeX Warning: Reference `alg:freight_IncrementCardinalityBlock' on page 75 und
efined on input line 355.


LaTeX Warning: Reference `theo:freight_sorting_correctness' on page 75 undefine
d on input line 357.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 75 undefined on input
 line 358.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_2' on page 75 undefined on input
 line 359.


LaTeX Warning: Reference `eq:freight_FREIGHT_E_1' on page 75 undefined on input
 line 360.


LaTeX Warning: Reference `eq:freight_FREIGHT' on page 75 undefined on input lin
e 360.

[75.93]

Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 408.


Package natbib Warning: Citation `alistarh2015streaming' on page 76 undefined o
n input line 411.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 411.


LaTeX Warning: Reference `subsec:Streaming Hypergraph Partitioning' on page 76 
undefined on input line 413.


Package natbib Warning: Citation `HYPE2018' on page 76 undefined on input line 
413.


Package natbib Warning: Citation `ccatalyurek2011patoh' on page 76 undefined on
 input line 413.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 416.


Package natbib Warning: Citation `schlag2016k' on page 76 undefined on input li
ne 419.


Overfull \hbox (14.46408pt too wide) in paragraph at lines 411--420
[]$\OT1/lmr/m/n/12 (-20) , $[]$, $[]$, $[]$, $[]$, $[]$, and $[]$.

LaTeX Warning: Reference `subsec:Hypergraphs' on page 76 undefined on input lin
e 427.

[76.94]

LaTeX Warning: Reference `fig:freight_connectivity_pp' on page 77 undefined on 
input line 510.


LaTeX Warning: Reference `fig:freight_cut_pp' on page 77 undefined on input lin
e 510.


LaTeX Warning: Reference `fig:freight_time_pp' on page 77 undefined on input li
ne 510.


LaTeX Warning: Reference `fig:freight_cut_pp' on page 77 undefined on input lin
e 510.


LaTeX Warning: Reference `fig:freight_cut_impr' on page 77 undefined on input l
ine 510.


Package natbib Warning: Citation `HYPE2018' on page 77 undefined on input line 
531.


Package natbib Warning: Citation `ccatalyurek2011patoh' on page 77 undefined on
 input line 531.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 77 undefined 
on input line 542.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 77 undefined 
on input line 544.

[77.95] [78.96 <./chapters/freight/Images/allhypergraphs_all_con/con/impr_chart
.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_con/con/pp_chart
.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/res/impr_cha
rt.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/res/pp_cha
rt.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_tim/tim/boxplo
t_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_tim/tim/p
p_chart.png (PNG copy)>]

LaTeX Warning: Reference `fig:freight_connectivity_impr' on page 79 undefined o
n input line 553.


LaTeX Warning: Reference `fig:freight_connectivity_pp' on page 79 undefined on 
input line 562.


LaTeX Warning: Reference `fig:freight_cut_impr' on page 79 undefined on input l
ine 569.


LaTeX Warning: Reference `fig:freight_cut_pp' on page 79 undefined on input lin
e 579.

[79.97]

LaTeX Warning: Reference `fig:freight_time_bp' on page 80 undefined on input li
ne 586.


Package natbib Warning: Citation `schlag2020high' on page 80 undefined on input
 line 590.


LaTeX Warning: Reference `fig:freight_time_pp' on page 80 undefined on input li
ne 593.


Package natbib Warning: Citation `StreamMultiSection' on page 80 undefined on i
nput line 613.

) [80.98]

LaTeX Warning: Reference `tab:streaming_hugeResults' on page 81 undefined on in
put line 31.


LaTeX Warning: Reference `sec:heistream_huge_graphs' on page 81 undefined on in
put line 32.


LaTeX Warning: Reference `sec:heistream_huge_graphs' on page 81 undefined on in
put line 33.


LaTeX Warning: Reference `sec:heistream_huge_graphs' on page 81 undefined on in
put line 35.


LaTeX Warning: Reference `subsec:Parameter Study' on page 81 undefined on input
 line 37.


LaTeX Warning: Reference `tab:streaming_hugeResults' on page 81 undefined on in
put line 38.


LaTeX Warning: Reference `tab:streaming_hugeResults' on page 81 undefined on in
put line 39.


LaTeX Warning: Reference `sec:heistream_huge_graphs' on page 81 undefined on in
put line 40.


LaTeX Warning: Float too large for page by 4.13483pt on input line 124.

[81.99] [82.100]
Underfull \vbox (badness 3657) has occurred while \output is active [83.101])
[84.102] (./chapters/chapter2.tex
Chapter 5.

Package natbib Warning: Citation `LocMotifClusHyperGraphPartition' on page 85 u
ndefined on input line 13.


Package natbib Warning: Citation `LocMotifClusHyperGraphPartitionExtAbs' on pag
e 85 undefined on input line 13.


Package natbib Warning: Citation `LocMotifClusMaxFlows' on page 85 undefined on
 input line 13.

(./chapters/lmcvhgp/chapter.tex [85.103]

LaTeX Warning: Reference `chap:lmcvhgp_Local Motif Clustering via (Hyper)Graph 
Partitioning' on page 86 undefined on input line 93.


Package natbib Warning: Citation `mqipaper2004' on page 86 undefined on input l
ine 93.


LaTeX Warning: Reference `fig:lmcvhgp_overall_algorithm' on page 86 undefined o
n input line 191.


LaTeX Warning: Reference `alg:lmcvhgp_overall_strategy' on page 86 undefined on
 input line 197.

[86.104]

Package natbib Warning: Citation `leskovec2009community' on page 87 undefined o
n input line 245.

[87.105 <./chapters/lmcvhgp/LocalMotifClustering.png (PNG copy)>]

Package natbib Warning: Citation `leskovec2009community' on page 88 undefined o
n input line 250.


Package natbib Warning: Citation `read1977graph' on page 88 undefined on input 
line 267.


Package natbib Warning: Citation `ortmann2014triangle' on page 88 undefined on 
input line 268.


Package natbib Warning: Citation `holme2002growing' on page 88 undefined on inp
ut line 269.


Package natbib Warning: Citation `batagelj2007short' on page 88 undefined on in
put line 269.


Package natbib Warning: Citation `prat2012shaping' on page 88 undefined on inpu
t line 269.


Package natbib Warning: Citation `kimmig2017shared' on page 88 undefined on inp
ut line 273.


Package natbib Warning: Citation `chiba1985arboricity' on page 88 undefined on 
input line 275.


Package natbib Warning: Citation `chiba1985arboricity' on page 88 undefined on 
input line 281.


LaTeX Warning: Reference `fig:lmcvhgp_model_construction' on page 88 undefined 
on input line 282.


LaTeX Warning: Reference `fig:lmcvhgp_model_construction_graph' on page 88 unde
fined on input line 282.


Underfull \vbox (badness 10000) has occurred while \output is active [88.106]

LaTeX Warning: Reference `fig:lmcvhgp_overall_algorithm' on page 89 undefined o
n input line 314.


LaTeX Warning: Reference `fig:lmcvhgp_model_construction' on page 89 undefined 
on input line 314.

[89.107]

LaTeX Warning: Reference `theo:lmcvhgp_cut_equivalence' on page 90 undefined on
 input line 329.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence' on page 90 unde
fined on input line 330.


Underfull \vbox (badness 10000) has occurred while \output is active [90.108 <.
/chapters/social/ModelConstruction.png (PNG copy)>]

LaTeX Warning: Reference `theo:lmcvhgp_cut_equivalence' on page 91 undefined on
 input line 365.

[91.109]

Package natbib Warning: Citation `benson2016higher' on page 92 undefined on inp
ut line 392.


Package natbib Warning: Citation `yin2017local' on page 92 undefined on input l
ine 392.


LaTeX Warning: Reference `fig:lmcvhgp_overall_algorithm' on page 92 undefined o
n input line 397.


LaTeX Warning: Reference `fig:lmcvhgp_model_construction_graph' on page 92 unde
fined on input line 397.

[92.110 <./chapters/lmcvhgp/SmallModelConstructionGraph.png (PNG copy)>]

LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph_complete' 
on page 93 undefined on input line 411.


Package natbib Warning: Citation `yin2017local' on page 93 undefined on input l
ine 411.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph' on page 9
3 undefined on input line 412.


LaTeX Warning: Reference `theo:lmcvhgp_cut_equivalence' on page 93 undefined on
 input line 414.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence' on page 93 unde
fined on input line 414.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph' on page 9
3 undefined on input line 415.


Package natbib Warning: Citation `benson2016higher' on page 93 undefined on inp
ut line 415.


Package natbib Warning: Citation `yin2017local' on page 93 undefined on input l
ine 420.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph_complete' 
on page 93 undefined on input line 437.


Underfull \vbox (badness 4120) has occurred while \output is active [93.111]

Package natbib Warning: Citation `schlag2016k' on page 94 undefined on input li
ne 454.


Package natbib Warning: Citation `kaHIPHomePage' on page 94 undefined on input 
line 455.


LaTeX Warning: Reference `fig:lmcvhgp_overall_algorithm' on page 94 undefined o
n input line 462.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph' on page 9
4 undefined on input line 476.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence' on page 94 unde
fined on input line 476.


Package natbib Warning: Citation `gottesburen2021scalable' on page 94 undefined
 on input line 482.


Package natbib Warning: Citation `gottesburen2021scalable' on page 94 undefined
 on input line 483.


Package natbib Warning: Citation `DBLP:conf/esa/GottesburenH00S21' on page 94 u
ndefined on input line 483.

[94.112]

Package natbib Warning: Citation `labelpropagationclustering' on page 95 undefi
ned on input line 488.

) (./chapters/social/chapter.tex

LaTeX Warning: Reference `subsec:lmcvhgp_Overall Strategy' on page 95 undefined
 on input line 138.


Package natbib Warning: Citation `mqipaper2004' on page 95 undefined on input l
ine 141.


LaTeX Warning: Reference `fig:social_overall_algorithm' on page 95 undefined on
 input line 145.


LaTeX Warning: Reference `alg:social_overall_strategy' on page 95 undefined on 
input line 149.

[95.113]

LaTeX Warning: Reference `subsec:lmcvhgp_Ball around Seed' on page 96 undefined
 on input line 191.


LaTeX Warning: Reference `subsec:lmcvhgp_Motif Enumeration' on page 96 undefine
d on input line 192.


LaTeX Warning: Reference `fig:social_model_construction' on page 96 undefined o
n input line 193.


LaTeX Warning: Reference `subsec:lmcvhgp_Hypergraph model' on page 96 undefined
 on input line 193.


LaTeX Warning: Reference `theo:social_conductance_equivalence' on page 96 undef
ined on input line 193.

[96.114 <./chapters/social/FlowLocalMotifClustering.png (PNG copy)>]

LaTeX Warning: Reference `fig:social_hyperedge_expansion' on page 97 undefined 
on input line 250.


LaTeX Warning: Reference `fig:social_flow_model' on page 97 undefined on input 
line 263.

[97.115]

LaTeX Warning: Reference `theo:social_flow_model_guarantee' on page 98 undefine
d on input line 268.


LaTeX Warning: Reference `theo:social_flow_model_guarantee' on page 98 undefine
d on input line 270.


LaTeX Warning: Reference `theo:social_conductance_equivalence' on page 98 undef
ined on input line 270.

[98.116 <./chapters/social/FlowModel.png (PNG copy)>]

Package natbib Warning: Citation `ford_fulkerson_1956' on page 99 undefined on 
input line 291.


LaTeX Warning: Reference `eq:social_forward_direction' on page 99 undefined on 
input line 308.


LaTeX Warning: Reference `eq:social_forward_direction_final' on page 99 undefin
ed on input line 308.


LaTeX Warning: Reference `theo:social_conductance_equivalence' on page 99 undef
ined on input line 309.


LaTeX Warning: Reference `eq:social_forward_direction_final' on page 99 undefin
ed on input line 309.


LaTeX Warning: Reference `eq:social_forward_direction_final' on page 99 undefin
ed on input line 326.


LaTeX Warning: Reference `eq:social_forward_direction_final' on page 99 undefin
ed on input line 327.


LaTeX Warning: Reference `eq:social_forward_direction' on page 99 undefined on 
input line 327.


Package natbib Warning: Citation `ford_fulkerson_1956' on page 99 undefined on 
input line 329.

[99.117]
Overfull \hbox (13.10965pt too wide) in paragraph at lines 333--342
[]\OT1/lmr/m/n/12 (-20) Now we show that the weights of the re-main-ing cut edg
es, i.e., edges from $\OML/lmm/m/it/12 B[]$ \OT1/lmr/m/n/12 (-20) to $[]$
[100.118]

Package natbib Warning: Citation `schlag2016k' on page 101 undefined on input l
ine 373.


Package natbib Warning: Citation `kaffpa' on page 101 undefined on input line 3
73.


Package natbib Warning: Citation `yin2017local' on page 101 undefined on input 
line 382.


Package natbib Warning: Citation `zhou2021high' on page 101 undefined on input 
line 383.


Package natbib Warning: Citation `zhang2019local' on page 101 undefined on inpu
t line 387.


LaTeX Warning: Reference `subsec:social_addcomp' on page 101 undefined on input
 line 388.


LaTeX Warning: Reference `tab:lmcvhgp_graphs' on page 101 undefined on input li
ne 394.


Package natbib Warning: Citation `yin2017local' on page 101 undefined on input 
line 396.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence' on page 101 und
efined on input line 406.


LaTeX Warning: Reference `theo:lmcvhgp_conductance_equivalence_graph' on page 1
01 undefined on input line 406.


LaTeX Warning: Reference `theo:social_flow_model_guarantee' on page 101 undefin
ed on input line 406.

[101.119]

LaTeX Warning: Reference `tab:lmcvhgp_graphs' on page 102 undefined on input li
ne 457.

[102.120]

LaTeX Warning: Reference `tab:lmcvhgp_graphs' on page 103 undefined on input li
ne 485.


LaTeX Warning: Reference `fig:social_SIMPLEstateoftheart_graph_res_pp' on page 
103 undefined on input line 486.


LaTeX Warning: Reference `fig:social_SIMPLEstateoftheart_graph_tim_pp' on page 
103 undefined on input line 486.


Package natbib Warning: Citation `yin2017local' on page 103 undefined on input 
line 486.


LaTeX Warning: Reference `tab:social_resultsoverall' on page 103 undefined on i
nput line 487.


LaTeX Warning: Reference `fig:social_SIMPLEstateoftheart_graph_res_pp' on page 
103 undefined on input line 491.


LaTeX Warning: Reference `tab:social_resultsoverall' on page 103 undefined on i
nput line 495.


LaTeX Warning: Reference `fig:social_SIMPLEstateoftheart_graph_tim_pp' on page 
103 undefined on input line 524.


LaTeX Warning: Reference `tab:social_resultsoverall' on page 103 undefined on i
nput line 529.

[103.121]

LaTeX Warning: Reference `fig:social_SIMPLEstateoftheart_graph_res_double' on p
age 104 undefined on input line 532.


Package natbib Warning: Citation `zhang2019local' on page 104 undefined on inpu
t line 554.


Package natbib Warning: Citation `zhang2019local' on page 104 undefined on inpu
t line 556.


LaTeX Warning: Reference `tab:social_resultsoverall' on page 104 undefined on i
nput line 560.

[104.122 <./chapters/social/plots/mqi_clique/res/pp_chart.png (PNG copy)>])
[105.123 <./chapters/social/plots/mqi_clique/res/double_chart.png (PNG copy)>])
[106.124] (./chapters/chapter3.tex
Chapter 6.

Package natbib Warning: Citation `HighQualityHierarchicalPM20' on page 107 unde
fined on input line 11.


Package natbib Warning: Citation `DistrMemMLevelSigGraphClustering_short' on pa
ge 107 undefined on input line 11.


Package natbib Warning: Citation `DistrMemMLevelSigGraphClustering' on page 107
 undefined on input line 11.

(./chapters/integratedProcessMappingPaper/chapter.tex [107.125]

LaTeX Warning: Reference `fig:intmap_multilevel' on page 108 undefined on input
 line 198.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
06.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
24.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
26.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
26.

[108.126 <./chapters/integratedProcessMappingPaper/MultilevelMap.png (PNG copy)
>]

Package natbib Warning: Citation `GlobalMultisection' on page 109 undefined on 
input line 259.


Package natbib Warning: Citation `schulz2017better' on page 109 undefined on in
put line 274.


Package natbib Warning: Citation `fiduccia1982lth' on page 109 undefined on inp
ut line 293.


Underfull \vbox (badness 10000) has occurred while \output is active [109.127]

LaTeX Warning: Reference `eq:process_mapping_obj' on page 110 undefined on inpu
t line 305.


Package natbib Warning: Citation `kaffpa' on page 110 undefined on input line 3
21.


Package natbib Warning: Citation `fiduccia1982lth' on page 110 undefined on inp
ut line 323.

[110.128]

Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
36.


Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
41.


Package natbib Warning: Citation `labelpropagationclustering' on page 111 undef
ined on input line 350.


Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
72.


Underfull \vbox (badness 6047) has occurred while \output is active [111.129]

LaTeX Warning: Reference `eq:bitsbinary' on page 112 undefined on input line 44
1.


LaTeX Warning: Reference `fig:bina_repr' on page 112 undefined on input line 44
1.

[112.130 <./chapters/integratedProcessMappingPaper/bin_rep.png (PNG copy)>]

Package natbib Warning: Citation `schlag2016k' on page 113 undefined on input l
ine 478.

[113.131]

Package natbib Warning: Citation `kaffpa' on page 114 undefined on input line 5
33.


Package natbib Warning: Citation `kaffpa' on page 114 undefined on input line 5
34.


Package natbib Warning: Citation `schulz2017better' on page 114 undefined on in
put line 535.


Package natbib Warning: Citation `muller2013optimale' on page 114 undefined on 
input line 538.


Package natbib Warning: Citation `schulz2017better' on page 114 undefined on in
put line 538.


Package natbib Warning: Citation `Scotch' on page 114 undefined on input line 5
39.


Package natbib Warning: Citation `GlobalMultisection' on page 114 undefined on 
input line 541.


Package natbib Warning: Citation `Scotch' on page 114 undefined on input line 5
44.


Package natbib Warning: Citation `walshaw2000mpm' on page 114 undefined on inpu
t line 547.


LaTeX Warning: Reference `tab:test_instances_walshaw' on page 114 undefined on 
input line 555.


LaTeX Warning: Reference `eq:process_mapping_obj' on page 114 undefined on inpu
t line 559.


Underfull \vbox (badness 2865) has occurred while \output is active [114.132]

LaTeX Warning: Reference `tab:test_instances_walshaw' on page 115 undefined on 
input line 594.


LaTeX Warning: Reference `tab:res_init_sol' on page 115 undefined on input line
 622.


LaTeX Warning: Reference `tab:res_init_sol' on page 115 undefined on input line
 627.


Package natbib Warning: Citation `schulz2017better' on page 115 undefined on in
put line 629.


LaTeX Warning: Reference `fig:InitSol' on page 115 undefined on input line 630.


[115.133] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmr.fd)

LaTeX Warning: Reference `fig:LSeco' on page 116 undefined on input line 710.

[116.134 <./chapters/integratedProcessMappingPaper/Results/InitSol/result.png (
PNG copy)> <./chapters/integratedProcessMappingPaper/Results/InitSol/time.png (
PNG copy)>]

LaTeX Warning: Reference `fig:LSeco' on page 117 undefined on input line 713.


LaTeX Warning: Reference `fig:DistMatrix' on page 117 undefined on input line 7
34.

[117.135]

LaTeX Warning: Reference `tab:test_instances_walshaw' on page 118 undefined on 
input line 774.


LaTeX Warning: Reference `fig:intmap_GenSol' on page 118 undefined on input lin
e 775.

[118.136 <./chapters/integratedProcessMappingPaper/Results/Refinement/result_ec
o.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/Refinement/
time_eco.png (PNG copy)>]
Overfull \hbox (8.57442pt too wide) in paragraph at lines 809--822
[]\OT1/lmr/m/n/12 (-20) We now high-light the com-par-i-son of var-i-ous con-fi
g-u-ra-tions/algorithms. $[]$
[119.137 <./chapters/integratedProcessMappingPaper/Results/DistMatrix/time_stro
ng.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/result_glo
b.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/time_glob.p
ng (PNG copy)>]) (./chapters/SignedClusterEvolutionaryPaper/chapter.tex

LaTeX Warning: Reference `fig:sgc_MSGC' on page 120 undefined on input line 222
.


LaTeX Warning: Reference `fig:sgc_MSGC_second_cycle' on page 120 undefined on i
nput line 222.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 120 unde
fined on input line 224.

[120.138]

LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 121 unde
fined on input line 257.


Package natbib Warning: Citation `labelpropagationclustering' on page 121 undef
ined on input line 261.

[121.139]

LaTeX Warning: Reference `fig:sgc_clustercontraction' on page 122 undefined on 
input line 273.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 122 unde
fined on input line 292.


LaTeX Warning: Reference `fig:sgc_clustercontraction' on page 122 undefined on 
input line 298.


Package natbib Warning: Citation `fiduccia1982lth' on page 122 undefined on inp
ut line 301.


Package natbib Warning: Citation `labelpropagationclustering' on page 122 undef
ined on input line 317.

[122.140]

Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
38.


Package natbib Warning: Citation `fiduccia1982lth' on page 123 undefined on inp
ut line 338.


Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
42.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 123 unde
fined on input line 359.


LaTeX Warning: Reference `fig:sgc_MSGC_second_cycle' on page 123 undefined on i
nput line 360.


Package natbib Warning: Citation `walshaw2004multilevel' on page 123 undefined 
on input line 363.


LaTeX Warning: Reference `sec:sgc_Distributed Evolutionary Signed Graph Cluster
ing' on page 123 undefined on input line 364.


Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
72.


Package natbib Warning: Citation `sanders2012distributed' on page 123 undefined
 on input line 381.

[123.141 <./chapters/SignedClusterEvolutionaryPaper/MSGC_second_cycle.png (PNG 
copy)>]

LaTeX Warning: Reference `alg:sgc_overall_evolutionary_strategy' on page 124 un
defined on input line 390.


Package natbib Warning: Citation `evolutionary_book' on page 124 undefined on i
nput line 400.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 124 unde
fined on input line 438.

[124.142]

Package natbib Warning: Citation `tournament_selection' on page 125 undefined o
n input line 457.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 125 unde
fined on input line 459.


LaTeX Warning: Reference `fig:sgc_recombination' on page 125 undefined on input
 line 460.


LaTeX Warning: Reference `fig:sgc_MSGC_second_cycle' on page 125 undefined on i
nput line 463.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 125 unde
fined on input line 475.


Underfull \vbox (badness 3219) has occurred while \output is active [125.143]

Package natbib Warning: Citation `sanders2012distributed' on page 126 undefined
 on input line 504.


LaTeX Warning: Reference `alg:sgc_overall_evolutionary_strategy' on page 126 un
defined on input line 505.


Package natbib Warning: Citation `randomgossip' on page 126 undefined on input 
line 506.


LaTeX Warning: Reference `alg:sgc_overall_evolutionary_strategy' on page 126 un
defined on input line 510.


Underfull \vbox (badness 10000) has occurred while \output is active [126.144 <
./chapters/SignedClusterEvolutionaryPaper/pics/recombination.png (PNG copy)>]

Package natbib Warning: Citation `bailoni2019generalized' on page 127 undefined
 on input line 530.


Package natbib Warning: Citation `bailoni2019generalized' on page 127 undefined
 on input line 531.


Package natbib Warning: Citation `keuper2015efficient' on page 127 undefined on
 input line 531.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 533.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 534.


LaTeX Warning: Reference `tab:sgc_graphs' on page 127 undefined on input line 5
39.


LaTeX Warning: Reference `tab:sgc_graphs' on page 127 undefined on input line 5
40.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 547.


LaTeX Warning: Reference `tab:sgc_graphs' on page 127 undefined on input line 5
48.

[127.145]

Package natbib Warning: Citation `sanders2012distributed' on page 128 undefined
 on input line 560.


LaTeX Warning: Reference `tab:sgc_graphs' on page 128 undefined on input line 5
68.


LaTeX Warning: Reference `alg:sgc_overall_multilevel_strategy' on page 128 unde
fined on input line 618.


LaTeX Warning: Reference `fig:sgc_convergence_overall' on page 128 undefined on
 input line 622.


LaTeX Warning: Reference `fig:sgc_convergence_individual' on page 128 undefined
 on input line 627.


LaTeX Warning: Reference `fig:sgc_convergence_overall' on page 128 undefined on
 input line 628.

[128.146]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `tbp') on input line 639.


LaTeX Warning: Reference `tab:sgc_results' on page 129 undefined on input line 
672.

[129.147 <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores
/conv/all/double_chart.png (PNG copy)>])
Underfull \vbox (badness 10000) has occurred while \output is active [130.148 <
./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores/conv/soc-
sign-Slashdot090216/double_chart.png (PNG copy)> <./chapters/SignedClusterEvolu
tionaryPaper/pics/convergence_1h_16cores/conv/soc-sign-epinions/double_chart.pn
g (PNG copy)> <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16
cores/conv/wikisigned-k2/double_chart.png (PNG copy)> <./chapters/SignedCluster
EvolutionaryPaper/pics/convergence_1h_16cores/conv/slashdot-zoo/double_chart.pn
g (PNG copy)>] [131.149]) [132.150] (./chapters/discussion.tex
Chapter 7.
[133.151]

LaTeX Warning: Reference `chap:Streaming Algorithms' on page 134 undefined on i
nput line 48.


LaTeX Warning: Reference `chap:Local Algorithms' on page 134 undefined on input
 line 48.


LaTeX Warning: Reference `chap:Multilevel Algorithms' on page 134 undefined on 
input line 48.

[134.152]) [135.153] [136.154]
No file main.bbl.
(./chapters/curriculum.tex
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmtt.fd) [137.155] [138.156
]) (./chapters/allpublications.tex [139.157] [140.158] [141.159])

Package natbib Warning: There were undefined citations.

(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-utf8.def)
(./main.aux (./chapters/abstracts.aux) (./chapters/acknowledgements.aux)
(./chapters/publications.aux) (./chapters/introduction.aux)
(./chapters/preliminaries.aux) (./chapters/related_work.aux)
(./chapters/chapter1.aux) (./chapters/chapter2.aux) (./chapters/chapter3.aux)
(./chapters/discussion.aux) (./chapters/curriculum.aux)
(./chapters/allpublications.aux))

LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `main.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information){/usr/local/texlive/2022/te
xmf-dist/fonts/enc/dvips/lm/lm-rmtt.enc}{/usr/local/texlive/2022/texmf-dist/fon
ts/enc/dvips/lm/lm-rm.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/l
m/lm-rmsc.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathit.
enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathsy.enc}{/usr/
local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathex.enc}</usr/local/texl
ive/2022/texmf-dist/fonts/type1/public/lm/lmbx10.pfb></usr/local/texlive/2022/t
exmf-dist/fonts/type1/public/lm/lmbx12.pfb></usr/local/texlive/2022/texmf-dist/
fonts/type1/public/lm/lmbx8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1
/public/lm/lmcsc10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/l
m/lmex10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi10.p
fb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi12.pfb></usr/l
ocal/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi6.pfb></usr/local/texliv
e/2022/texmf-dist/fonts/type1/public/lm/lmmi8.pfb></usr/local/texlive/2022/texm
f-dist/fonts/type1/public/lm/lmr10.pfb></usr/local/texlive/2022/texmf-dist/font
s/type1/public/lm/lmr12.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/pub
lic/lm/lmr17.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr6
.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr7.pfb></usr/l
ocal/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr8.pfb></usr/local/texlive
/2022/texmf-dist/fonts/type1/public/lm/lmri12.pfb></usr/local/texlive/2022/texm
f-dist/fonts/type1/public/lm/lmss10.pfb></usr/local/texlive/2022/texmf-dist/fon
ts/type1/public/lm/lmss12.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/p
ublic/lm/lmss8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lm
sy10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmsy6.pfb></
usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmsy8.pfb></usr/local/t
exlive/2022/texmf-dist/fonts/type1/public/lm/lmtt12.pfb></usr/local/texlive/202
2/texmf-dist/fonts/type1/public/amsfonts/symbols/msbm10.pfb>
Output written on main.pdf (159 pages, 9617970 bytes).
SyncTeX written on main.synctex.gz.
Transcript written on main.log.
This is BibTeX, Version 0.99d (TeX Live 2022)
The top-level auxiliary file: main.aux
The style file: unsrtnat.bst
Database file #1: bibliography.bib
Warning--empty publisher in sastry2014genetic
Warning--empty publisher in benchmarksfornetworksanalysis
Warning--empty year in Scotch
Warning--empty publisher in Walshaw07
Warning--empty year in kaHIPHomePage
Warning--empty year in viemaWebsite
Warning--empty year in LocMotifClusHyperGraphPartition
Warning--empty year in LocMotifClusHyperGraphPartition
(There were 8 warnings)
This is pdfTeX, Version 3.141592653-2.6-1.40.24 (TeX Live 2022) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2021-11-15> patch level 1
L3 programming layer <2022-02-24> (./hdphdthesis.cls
Document Class: hdphdthesis 08 Jan 2022 Heidelberg University Dr. rer. nat. The
sis class
(/usr/local/texlive/2022/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/book.cls
Document Class: book 2021/10/04 v1.4n Standard LaTeX document class
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/bk12.clo))
(/usr/local/texlive/2022/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-li
sts.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.c
ode.tex))) (/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/sttools/stfloats.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/emptypage/emptypage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/array.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/lmodern.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/placeins/placeins.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algpseudocode.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algorithmicx.sty
Document Style algorithmicx 1.2 - a greatly improved `algorithmic' style
)
Document Style - pseudocode environments for use with the `algorithmicx' style
) (/usr/local/texlive/2022/texmf-dist/tex/latex/numprint/numprint.sty
No configuration file `numprint.cfg' found.)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2022/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2022/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.
tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothan
dlers.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytopaths.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarypositioning.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/threeparttable/threeparttable.sty
) (/usr/local/texlive/2022/texmf-dist/tex/latex/hvfloat/hvfloat.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/picture/picture.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multido/multido.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/multido/multido.tex
 v1.42, 2010/05/14 <tvz>)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/natbib/natbib.sty

Package natbib Warning: The `cite' package should not be used
(natbib)                with natbib. Use option `sort' instead.

) (/usr/local/texlive/2022/texmf-dist/tex/latex/doi/doi.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.arrows.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.arrows.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarychains.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathreplacing.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduledecoration
s.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathreplacing.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/framed/framed.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xifthen/xifthen.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense-english.ldf
)) (/usr/local/texlive/2022/texmf-dist/tex/latex/ccicons/ccicons.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmr.fd)

LaTeX Warning: Unused global option(s):
    [mathcomp,marginleft,marginright,margintop,marginbottom,bindingoffset].

(./main.aux (./chapters/abstracts.aux) (./chapters/acknowledgements.aux)
(./chapters/publications.aux) (./chapters/introduction.aux)
(./chapters/preliminaries.aux) (./chapters/related_work.aux)
(./chapters/chapter1.aux) (./chapters/chapter2.aux

LaTeX Warning: Label `sec:lmcvhgp_Local Motif Clustering via (Hyper)Graph Parti
tioning' multiply defined.

) (./chapters/chapter3.aux

LaTeX Warning: Label `subsec:Parameter Study' multiply defined.


LaTeX Warning: Label `sec:sgc_Multilevel Signed Graph Clustering' multiply defi
ned.

) (./chapters/discussion.aux) (./chapters/curriculum.aux)
(./chapters/allpublications.aux))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/ltcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2022/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./main.out) (./main.out)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omllmm.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmsy.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omxlmex.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msb.cfg) [1.1{/usr/l
ocal/texlive/2022/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2.2] [3.3]
[4.4] (./chapters/abstracts.tex [5.5] [6.6]
Underfull \hbox (badness 5696) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Dis-ser-ta-tion be-fasst sich mit der Un-ter-suchung ver-
schiedener Arten von

Underfull \hbox (badness 6708) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Multi-Level-Algorithmen. Im Bere-ich der Streaming-Algori
thmen leis-ten

Underfull \hbox (badness 10000) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) wir Beitr^^?age mit hochef-fizien-ten und ef-fek-tiven Al
-go-rith-men f^^?ur die
[7.7]) (./chapters/acknowledgements.tex [8.8]
Underfull \vbox (badness 1533) has occurred while \output is active [9.9]
Underfull \vbox (badness 1515) has occurred while \output is active [10.10]
[11.11]) (./chapters/publications.tex [12.12]
Underfull \hbox (badness 10000) in paragraph at lines 2--3

[13.13] [14.14] [15.15]) [16.16] (./main.toc [17.17] [18.18]) [19.19] [20.20]
(./chapters/introduction.tex
Chapter 1.

Package natbib Warning: Citation `Garey1974' on page 1 undefined on input line 
32.


Package natbib Warning: Citation `BuiJ92' on page 1 undefined on input line 32.



Package natbib Warning: Citation `tsourakakis2014fennel' on page 1 undefined on
 input line 34.


Package natbib Warning: Citation `awadelkarim2020prioritized' on page 1 undefin
ed on input line 34.


Package natbib Warning: Citation `jafari2021fast' on page 1 undefined on input 
line 34.


Package natbib Warning: Citation `mayer2018adwise' on page 1 undefined on input
 line 34.


Package natbib Warning: Citation `hoang2019cusp' on page 1 undefined on input l
ine 34.


Package natbib Warning: Citation `alistarh2015streaming' on page 1 undefined on
 input line 34.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 1 undefined o
n input line 34.


Package natbib Warning: Citation `HeiStream' on page 1 undefined on input line 
34.


Package natbib Warning: Citation `StreamMultiSection' on page 1 undefined on in
put line 34.


Package natbib Warning: Citation `freight_paper' on page 1 undefined on input l
ine 34.

[1.21]

Package natbib Warning: Citation `kannan2004clusterings' on page 2 undefined on
 input line 49.


Package natbib Warning: Citation `epasto2014reduce' on page 2 undefined on inpu
t line 51.


Package natbib Warning: Citation `jeub2015think' on page 2 undefined on input l
ine 51.


Package natbib Warning: Citation `voevodski2009spectral' on page 2 undefined on
 input line 51.


Package natbib Warning: Citation `wagner1993between' on page 2 undefined on inp
ut line 52.


Package natbib Warning: Citation `andersen2006local' on page 2 undefined on inp
ut line 54.


Package natbib Warning: Citation `leskovec2009community' on page 2 undefined on
 input line 54.


Package natbib Warning: Citation `chung2013solving' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `li2015uncovering' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `fountoulakis2020flowbased' on page 2 undefine
d on input line 54.


Package natbib Warning: Citation `yin2017local' on page 2 undefined on input li
ne 54.


Package natbib Warning: Citation `zhang2019local' on page 2 undefined on input 
line 54.


Package natbib Warning: Citation `meng2019local' on page 2 undefined on input l
ine 54.


Package natbib Warning: Citation `murali2020online' on page 2 undefined on inpu
t line 54.


Package natbib Warning: Citation `yin2017local' on page 2 undefined on input li
ne 55.


Underfull \vbox (badness 10000) has occurred while \output is active [2.22]

Package natbib Warning: Citation `kannan2004clusterings' on page 3 undefined on
 input line 63.


Package natbib Warning: Citation `brandes2007modularity' on page 3 undefined on
 input line 63.


Package natbib Warning: Citation `application_review' on page 3 undefined on in
put line 69.


Package natbib Warning: Citation `DBLP:phd/dnb/Wakabayashi86' on page 3 undefin
ed on input line 70.

[3.23] [4.24] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmss.fd)

Package natbib Warning: Citation `mqipaper2004' on page 5 undefined on input li
ne 133.

[5.25] [6.26]) [7.27] (./chapters/preliminaries.tex [8.28]
Chapter 2.
[9.29]

Package natbib Warning: Citation `brandes2007modularity' on page 10 undefined o
n input line 78.


Package natbib Warning: Citation `kannan2004clusterings' on page 10 undefined o
n input line 78.


Package natbib Warning: Citation `benson2016higher' on page 10 undefined on inp
ut line 82.

[10.30]

Package natbib Warning: Citation `brandfass2013rank' on page 11 undefined on in
put line 105.

[11.31]

Package natbib Warning: Citation `ford_fulkerson_1956' on page 12 undefined on 
input line 143.

[12.32]

Package natbib Warning: Citation `push_relabel88' on page 13 undefined on input
 line 149.


Package natbib Warning: Citation `veldt2022hypergraph' on page 13 undefined on 
input line 155.


Package natbib Warning: Citation `lawler1973cutsets' on page 13 undefined on in
put line 155.


Underfull \vbox (badness 10000) has occurred while \output is active [13.33]
[14.34 <./chapters/social/HyperEdgeExpansions.png (PNG copy)>]

Package natbib Warning: Citation `kaffpa' on page 15 undefined on input line 20
0.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 15 undefi
ned on input line 213.


Package natbib Warning: Citation `evolutionary_book' on page 15 undefined on in
put line 230.


Package natbib Warning: Citation `sastry2014genetic' on page 15 undefined on in
put line 231.


Package natbib Warning: Citation `goldberg1989messy' on page 15 undefined on in
put line 233.


Package natbib Warning: Citation `Michalewicz:1996:GAD:229930' on page 15 undef
ined on input line 234.

[15.35 <./chapters/heistream/pics/MGP.png (PNG copy)> <./chapters/SignedCluster
EvolutionaryPaper/pics/cluster_contraction.png (PNG copy)>]
Underfull \vbox (badness 10000) has occurred while \output is active [16.36 <./
chapters/SignedClusterEvolutionaryPaper/pics/LP_illustration.png (PNG copy)>]

Package natbib Warning: Citation `snapnets' on page 17 undefined on input line 
287.


Package natbib Warning: Citation `nr-aaai15' on page 17 undefined on input line
 287.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 287.


Package natbib Warning: Citation `kappa' on page 17 undefined on input line 287
.


Package natbib Warning: Citation `funke2019communication' on page 17 undefined 
on input line 287.


Package natbib Warning: Citation `snapnets' on page 17 undefined on input line 
289.


Package natbib Warning: Citation `nr-aaai15' on page 17 undefined on input line
 289.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 290.


Package natbib Warning: Citation `kappa' on page 17 undefined on input line 294
.


Package natbib Warning: Citation `funke2019communication' on page 17 undefined 
on input line 295.


Package natbib Warning: Citation `DBLP:journals/corr/abs-2003-00736' on page 17
 undefined on input line 295.


Package natbib Warning: Citation `soper2004combined' on page 17 undefined on in
put line 388.


Package natbib Warning: Citation `davis2011university' on page 17 undefined on 
input line 389.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 17 und
efined on input line 390.


Package natbib Warning: Citation `DSSW09' on page 17 undefined on input line 39
3.

[17.37 <./chapters/more_recent_partitioning_survey/img/streaming/streaming.png 
(PNG copy)>]

Package natbib Warning: Citation `snapnets' on page 18 undefined on input line 
505.


Package natbib Warning: Citation `nr-aaai15' on page 18 undefined on input line
 505.


Package natbib Warning: Citation `benchmarksfornetworksanalysis' on page 18 und
efined on input line 505.


Package natbib Warning: Citation `yin2017local' on page 18 undefined on input l
ine 509.

[18.38]

Package natbib Warning: Citation `schlag2016k' on page 19 undefined on input li
ne 520.


Package natbib Warning: Citation `alpert1998ispd98' on page 19 undefined on inp
ut line 522.


Package natbib Warning: Citation `davis2011university' on page 19 undefined on 
input line 523.


Package natbib Warning: Citation `Belov2014' on page 19 undefined on input line
 524.


Package natbib Warning: Citation `snap' on page 19 undefined on input line 534.



Package natbib Warning: Citation `konect' on page 19 undefined on input line 53
4.


Underfull \vbox (badness 10000) has occurred while \output is active [19.39]
[20.40] [21.41 <./chapters/social/plots/mqi_clique/tim/pp_chart.png (PNG copy)>
]) [22.42] (./chapters/related_work.tex
Chapter 3.

Package natbib Warning: Citation `ccatalyurek2011patoh' on page 23 undefined on
 input line 13.


Package natbib Warning: Citation `parmetis-conference' on page 23 undefined on 
input line 13.


Package natbib Warning: Citation `hMetis' on page 23 undefined on input line 13
.


Package natbib Warning: Citation `Pellegrini96experimentalanalysis' on page 23 
undefined on input line 13.


Package natbib Warning: Citation `HYPE2018' on page 23 undefined on input line 
13.


Package natbib Warning: Citation `kabapeE' on page 23 undefined on input line 1
3.


Package natbib Warning: Citation `gottesburen2021deep' on page 23 undefined on 
input line 13.


Package natbib Warning: Citation `schlag2016k' on page 23 undefined on input li
ne 13.


Package natbib Warning: Citation `mt-kahypar-d' on page 23 undefined on input l
ine 13.


Package natbib Warning: Citation `DBLP:conf/europar/Akhremtsev0018' on page 23 
undefined on input line 13.


Package natbib Warning: Citation `more_recent_advances_hgp' on page 23 undefine
d on input line 14.


Package natbib Warning: Citation `SPPGPOverviewPaper' on page 23 undefined on i
nput line 14.


Package natbib Warning: Citation `DBLP:reference/bdt/0003S19' on page 23 undefi
ned on input line 14.


Package natbib Warning: Citation `stanton2012streaming' on page 23 undefined on
 input line 26.

[23.43]

Package natbib Warning: Citation `stanton2014streaming' on page 24 undefined on
 input line 38.


Package natbib Warning: Citation `chung2003generalizations' on page 24 undefine
d on input line 40.


Package natbib Warning: Citation `tsourakakis2014fennel' on page 24 undefined o
n input line 42.


Package natbib Warning: Citation `brandes2007modularity' on page 24 undefined o
n input line 43.


Package natbib Warning: Citation `stanton2012streaming' on page 24 undefined on
 input line 49.


Package natbib Warning: Citation `zhang2018akin' on page 24 undefined on input 
line 54.


Package natbib Warning: Citation `hamers1989similarity' on page 24 undefined on
 input line 57.


Package natbib Warning: Citation `nishimura2013restreaming' on page 24 undefine
d on input line 73.


Package natbib Warning: Citation `stanton2012streaming' on page 24 undefined on
 input line 77.


Package natbib Warning: Citation `tsourakakis2014fennel' on page 24 undefined o
n input line 77.

[24.44]

Package natbib Warning: Citation `awadelkarim2020prioritized' on page 25 undefi
ned on input line 86.


Package natbib Warning: Citation `patwary2019window' on page 25 undefined on in
put line 97.


Package natbib Warning: Citation `jafari2021fast' on page 25 undefined on input
 line 102.

[25.45]

Package natbib Warning: Citation `alistarh2015streaming' on page 26 undefined o
n input line 119.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 26 undefined 
on input line 128.


Package natbib Warning: Citation `alistarh2015streaming' on page 26 undefined o
n input line 128.

[26.46]

Package natbib Warning: Citation `benson2015tensor' on page 27 undefined on inp
ut line 201.


Package natbib Warning: Citation `yin2017local' on page 27 undefined on input l
ine 201.


Package natbib Warning: Citation `klymko2014using' on page 27 undefined on inpu
t line 201.


Package natbib Warning: Citation `prvzulj2007biological' on page 27 undefined o
n input line 201.


Package natbib Warning: Citation `tsourakakis2017scalable' on page 27 undefined
 on input line 201.


Package natbib Warning: Citation `kloster2014heat' on page 27 undefined on inpu
t line 203.


Package natbib Warning: Citation `li2015uncovering' on page 27 undefined on inp
ut line 203.


Package natbib Warning: Citation `mahoney2012local' on page 27 undefined on inp
ut line 203.


Package natbib Warning: Citation `cui2014local' on page 27 undefined on input l
ine 203.


Package natbib Warning: Citation `sozio2010community' on page 27 undefined on i
nput line 203.

[27.47]

Package natbib Warning: Citation `rohe2013blessing' on page 28 undefined on inp
ut line 210.


Package natbib Warning: Citation `huang2014querying' on page 28 undefined on in
put line 213.


Package natbib Warning: Citation `cohen2008trusses' on page 28 undefined on inp
ut line 213.


Package natbib Warning: Citation `yin2017local' on page 28 undefined on input l
ine 217.


Package natbib Warning: Citation `zhang2019local' on page 28 undefined on input
 line 224.


Package natbib Warning: Citation `meng2019local' on page 28 undefined on input 
line 231.


Underfull \vbox (badness 3657) has occurred while \output is active [28.48]

Package natbib Warning: Citation `zhou2021high' on page 29 undefined on input l
ine 238.


Package natbib Warning: Citation `spielman2013local' on page 29 undefined on in
put line 241.


Package natbib Warning: Citation `shang2022local' on page 29 undefined on input
 line 245.


Package natbib Warning: Citation `DBLP:journals/fgcs/WalshawC01' on page 29 und
efined on input line 267.


Package natbib Warning: Citation `DBLP:conf/hpcn/PellegriniR96' on page 29 unde
fined on input line 267.


Package natbib Warning: Citation `schulz2017better' on page 29 undefined on inp
ut line 268.


Package natbib Warning: Citation `brandfass2013rank' on page 29 undefined on in
put line 268.


Package natbib Warning: Citation `heider1972computationally' on page 29 undefin
ed on input line 268.


Package natbib Warning: Citation `muller2013optimale' on page 29 undefined on i
nput line 268.


Package natbib Warning: Citation `glantz2015algorithms' on page 29 undefined on
 input line 268.


Package natbib Warning: Citation `GPOverviewBook' on page 29 undefined on input
 line 274.


Package natbib Warning: Citation `SPPGPOverviewPaper' on page 29 undefined on i
nput line 274.

[29.49]

Package natbib Warning: Citation `muller2013optimale' on page 30 undefined on i
nput line 289.


Package natbib Warning: Citation `heider1972computationally' on page 30 undefin
ed on input line 294.


Package natbib Warning: Citation `brandfass2013rank' on page 30 undefined on in
put line 299.


Package natbib Warning: Citation `DBLP:conf/ipps/DeveciKUC15' on page 30 undefi
ned on input line 304.


Package natbib Warning: Citation `Scotch' on page 30 undefined on input line 31
0.


Package natbib Warning: Citation `Walshaw07' on page 30 undefined on input line
 310.


Package natbib Warning: Citation `8666156' on page 30 undefined on input line 3
14.


Package natbib Warning: Citation `DBLP:journals/tpds/DeveciRDC16' on page 30 un
defined on input line 316.


Underfull \vbox (badness 1515) has occurred while \output is active [30.50]

Package natbib Warning: Citation `vogelstein2015fast' on page 31 undefined on i
nput line 322.


Package natbib Warning: Citation `umeyama1988eigendecomposition' on page 31 und
efined on input line 326.


Package natbib Warning: Citation `singh2007pairwise' on page 31 undefined on in
put line 326.


Package natbib Warning: Citation `zaslavskiy2008path' on page 31 undefined on i
nput line 326.


Package natbib Warning: Citation `burkard1997qaplib' on page 31 undefined on in
put line 326.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 331.


Package natbib Warning: Citation `muller2013optimale' on page 31 undefined on i
nput line 334.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 335.


Package natbib Warning: Citation `glantz2018topology' on page 31 undefined on i
nput line 338.


Package natbib Warning: Citation `Scotch' on page 31 undefined on input line 34
2.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 342.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 349.


Package natbib Warning: Citation `kaHIPHomePage' on page 31 undefined on input 
line 350.


Package natbib Warning: Citation `brandfass2013rank' on page 31 undefined on in
put line 353.


Package natbib Warning: Citation `muller2013optimale' on page 31 undefined on i
nput line 355.


Package natbib Warning: Citation `Walshaw07' on page 31 undefined on input line
 355.


Package natbib Warning: Citation `glantz2015algorithms' on page 31 undefined on
 input line 355.


Package natbib Warning: Citation `GlobalMultisection' on page 31 undefined on i
nput line 356.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 356.


Package natbib Warning: Citation `schulz2017better' on page 31 undefined on inp
ut line 358.


Underfull \vbox (badness 1515) has occurred while \output is active [31.51]

Package natbib Warning: Citation `PredariProcessMapping21' on page 32 undefined
 on input line 366.


Package natbib Warning: Citation `parmetis-conference' on page 32 undefined on 
input line 370.


Package natbib Warning: Citation `DBLP:journals/tpds/MeyerhenkeSS17' on page 32
 undefined on input line 370.


Package natbib Warning: Citation `von2020efficient' on page 32 undefined on inp
ut line 377.


Package natbib Warning: Citation `viemaWebsite' on page 32 undefined on input l
ine 384.


Package natbib Warning: Citation `yang2007community' on page 32 undefined on in
put line 400.


Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 32 unde
fined on input line 400.


Package natbib Warning: Citation `traag2009community' on page 32 undefined on i
nput line 400.


Package natbib Warning: Citation `correlationclustering_overall' on page 32 und
efined on input line 400.


Package natbib Warning: Citation `demaine2006correlation' on page 32 undefined 
on input line 400.


Package natbib Warning: Citation `grotschel1989cutting' on page 32 undefined on
 input line 400.


Package natbib Warning: Citation `dinh2015toward' on page 32 undefined on input
 line 400.


Package natbib Warning: Citation `miyauchi2015redundant' on page 32 undefined o
n input line 400.


Package natbib Warning: Citation `miyauchi2018exact' on page 32 undefined on in
put line 400.


Package natbib Warning: Citation `kunegis2010spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `gallier2016spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `knyazev2018spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `mercado2019spectral' on page 32 undefined on 
input line 401.


Package natbib Warning: Citation `he2011ant' on page 32 undefined on input line
 401.


Package natbib Warning: Citation `zhu2018novel' on page 32 undefined on input l
ine 401.


Package natbib Warning: Citation `brusco2019partitioning' on page 32 undefined 
on input line 401.


Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 32 unde
fined on input line 401.


Package natbib Warning: Citation `abdulrahman2020enhanced' on page 32 undefined
 on input line 401.


Package natbib Warning: Citation `chen2022iterated' on page 32 undefined on inp
ut line 401.


Package natbib Warning: Citation `gallier2016spectral' on page 32 undefined on 
input line 402.


Package natbib Warning: Citation `surveyTangCAL16' on page 32 undefined on inpu
t line 402.


Package natbib Warning: Citation `tomasso2021advances' on page 32 undefined on 
input line 402.

[32.52]

Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 429.


Package natbib Warning: Citation `bailoni2019generalized' on page 33 undefined 
on input line 431.


Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 432.


Package natbib Warning: Citation `keuper2015efficient' on page 33 undefined on 
input line 440.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 33 undefined on in
put line 444.

[33.53]

Package natbib Warning: Citation `memeticsiggraphcommdetec2020' on page 34 unde
fined on input line 454.


Package natbib Warning: Citation `gomez2009analysis' on page 34 undefined on in
put line 455.


Underfull \vbox (badness 10000) has occurred while \output is active [34.54]

Package natbib Warning: Citation `grotschel1989cutting' on page 35 undefined on
 input line 471.


Package natbib Warning: Citation `dinh2015toward' on page 35 undefined on input
 line 473.


Package natbib Warning: Citation `grotschel1989cutting' on page 35 undefined on
 input line 473.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 473.


Package natbib Warning: Citation `dinh2015toward' on page 35 undefined on input
 line 473.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 474.


Package natbib Warning: Citation `miyauchi2018exact' on page 35 undefined on in
put line 476.


Package natbib Warning: Citation `miyauchi2015redundant' on page 35 undefined o
n input line 476.


Package natbib Warning: Citation `koshimura2022concise' on page 35 undefined on
 input line 478.


Package natbib Warning: Citation `miyauchi2018exact' on page 35 undefined on in
put line 478.

[35.55]) [36.56] (./chapters/chapter1.tex
Chapter 4.

Package natbib Warning: Citation `HeiStream' on page 37 undefined on input line
 17.


Package natbib Warning: Citation `StreamMultiSection' on page 37 undefined on i
nput line 17.


Package natbib Warning: Citation `freight_paper' on page 37 undefined on input 
line 17.

(./chapters/heistream/chapter.tex
Underfull \vbox (badness 10000) has occurred while \output is active [37.57]
[38.58]
Underfull \vbox (badness 10000) has occurred while \output is active [39.59 <./
chapters/heistream/MultilevelBufferedStreamGP.png (PNG copy)>]

Package natbib Warning: Citation `tsourakakis2014fennel' on page 40 undefined o
n input line 251.

[40.60] [41.61]

Package natbib Warning: Citation `kaffpa' on page 42 undefined on input line 30
7.


Package natbib Warning: Citation `karypis1998fast' on page 42 undefined on inpu
t line 308.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 42 undefi
ned on input line 316.


Package natbib Warning: Citation `labelpropagationclustering' on page 42 undefi
ned on input line 324.


Package natbib Warning: Citation `pcomplexnetworksviacluster' on page 42 undefi
ned on input line 324.

[42.62]
Underfull \vbox (badness 10000) has occurred while \output is active [43.63]
[44.64]

Package natbib Warning: Citation `jafari2021fast' on page 45 undefined on input
 line 433.


Package natbib Warning: Citation `jafari2021fast' on page 45 undefined on input
 line 435.

[45.65] [46.66] [47.67 <./chapters/heistream/Images/repetitions_label_prop/res_
rep_label.png (PNG copy)> <./chapters/heistream/Images/tim_TIMErep_label/tim_TI
MErep_label.png (PNG copy)> <./chapters/heistream/Images/StopRule/res_StopRule.
png (PNG copy)> <./chapters/heistream/Images/restream/res_restream.png (PNG cop
y)> <./chapters/heistream/Images/batch_noFennel/res_batch_noFennel.png (PNG cop
y)> <./chapters/heistream/Images/tim_TIMEbatch_noFennel/tim_TIMEbatch_noFennel.
png (PNG copy)>]
Underfull \vbox (badness 1348) has occurred while \output is active [48.68 <./c
hapters/heistream/Images/ghost/res_ghost.png (PNG copy)> <./chapters/heistream/
Images/tim_TIMEghost/tim_TIMEghost.png (PNG copy)>]
Overfull \hbox (11.6059pt too wide) in paragraph at lines 665--701
 [][] 
[49.69 <./chapters/heistream/Images/MultiLDG/comparison_MultiLDG_vertical/Multi
LDGFullBuffer.png (PNG copy)>] [50.70]

Package natbib Warning: Citation `karypis1998fast' on page 51 undefined on inpu
t line 778.


Package natbib Warning: Citation `kaffpa' on page 51 undefined on input line 77
8.

[51.71 <./chapters/heistream/Images/res_stateOfTheArtPlots/res_stateOfTheArtPlo
ts.png (PNG copy)> <./chapters/heistream/Images/tim_stateOfTheArtPlots/tim_stat
eOfTheArtPlots.png (PNG copy)> <./chapters/heistream/Images/res_stateOfTheArtPl
ots/pp_res_stateOfTheArtPlots.png (PNG copy)> <./chapters/heistream/Images/tim_
stateOfTheArtPlots/pp_tim_stateOfTheArtPlots.png (PNG copy)>]

Package natbib Warning: Citation `jafari2021fast' on page 52 undefined on input
 line 798.


Underfull \vbox (badness 5939) has occurred while \output is active [52.72 <./c
hapters/heistream/Images/res_restreamStateOfTheArtPlots/pp_res_restreamStateOfT
heArtPlots.png (PNG copy)>] [53.73] [54.74 <./chapters/heistream/Visualization.
png (PNG copy)>]
Overfull \hbox (0.9859pt too wide) in paragraph at lines 867--940
 [][] 

LaTeX Warning: Float too large for page by 23.98486pt on input line 942.

[55.75] [56.76]) (./chapters/recmultisec/chapter.tex

Package natbib Warning: Citation `schulz2017better' on page 57 undefined on inp
ut line 124.


Package natbib Warning: Citation `GlobalMultisection' on page 57 undefined on i
nput line 124.


Package natbib Warning: Citation `GlobalMultisection' on page 57 undefined on i
nput line 131.

[57.77]
Underfull \vbox (badness 2012) has occurred while \output is active [58.78]
[59.79 <./chapters/recmultisec/Multi-Section.png (PNG copy)>] [60.80]

Package natbib Warning: Citation `more_recent_advances_hgp' on page 61 undefine
d on input line 298.

[61.81] [62.82]
Underfull \vbox (badness 10000) has occurred while \output is active [63.83]

Package natbib Warning: Citation `tsourakakis2014fennel' on page 64 undefined o
n input line 431.


Package natbib Warning: Citation `gottesburen2021deep' on page 64 undefined on 
input line 436.


Package natbib Warning: Citation `schulz2017better' on page 64 undefined on inp
ut line 449.


Package natbib Warning: Citation `GlobalMultisection' on page 64 undefined on i
nput line 449.

[64.84]
Overfull \hbox (0.77881pt too wide) in paragraph at lines 798--799
\OT1/lmr/m/n/12 (-20) In this sec-tion, we show ex-per-i-ments in which we com-
pare $[]$
[65.85] [66.86 <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/chart
.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/pp_
chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/re
s/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/
tim/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateofthear
tPar/GP/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoft
heartPar/tim/chart.png (PNG copy)>] [67.87 <./chapters/recmultisec/Images/tunin
g/parallelSpeedups/speedup/soc-orkut-dir/chart.png (PNG copy)> <./chapters/recm
ultisec/Images/tuning/parallelSpeedups/times/soc-orkut-dir/chart.png (PNG copy)
> <./chapters/recmultisec/Images/tuning/parallelSpeedups/speedup/HV15R/chart.pn
g (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/times/HV15
R/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/
speedup/soc-LiveJournal1/chart.png (PNG copy)> <./chapters/recmultisec/Images/t
uning/parallelSpeedups/times/soc-LiveJournal1/chart.png (PNG copy)>] [68.88]

Package natbib Warning: Citation `gottesburen2021deep' on page 69 undefined on 
input line 900.

) (./chapters/freight/chapter.tex [69.89] [70.90]
Overfull \hbox (10.08015pt too wide) in paragraph at lines 181--185
\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m/it/12 V[]\OT1/lmr/m/n/12 (-
20) )[]$, where the weight $\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m
/it/12 v\OT1/lmr/m/n/12 (-20) )$ of $\OML/lmm/m/it/12 v$ \OT1/lmr/m/n/12 (-20) 
is []. 

Package natbib Warning: Citation `alistarh2015streaming' on page 71 undefined o
n input line 209.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 71 undefined 
on input line 209.

[71.91 <./chapters/freight/streaming.png (PNG copy)>] [72.92]
Underfull \vbox (badness 1694) has occurred while \output is active [73.93 <./c
hapters/freight/DecomposeEqFREIGHT.png (PNG copy)>]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `htbp') on input line 305.

[74.94 <./chapters/freight/SortingArrays.png (PNG copy)>] [75.95]

Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 408.


Package natbib Warning: Citation `alistarh2015streaming' on page 76 undefined o
n input line 411.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 411.


Package natbib Warning: Citation `HYPE2018' on page 76 undefined on input line 
413.


Package natbib Warning: Citation `ccatalyurek2011patoh' on page 76 undefined on
 input line 413.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 76 undefined 
on input line 416.


Package natbib Warning: Citation `schlag2016k' on page 76 undefined on input li
ne 419.


Overfull \hbox (14.46408pt too wide) in paragraph at lines 411--420
[]$\OT1/lmr/m/n/12 (-20) , $[]$, $[]$, $[]$, $[]$, $[]$, and $[]$.
[76.96]

Package natbib Warning: Citation `HYPE2018' on page 77 undefined on input line 
531.


Package natbib Warning: Citation `ccatalyurek2011patoh' on page 77 undefined on
 input line 531.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 77 undefined 
on input line 542.


Package natbib Warning: Citation `tacsyaran2021streaming' on page 77 undefined 
on input line 544.

[77.97] [78.98 <./chapters/freight/Images/allhypergraphs_all_con/con/impr_chart
.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_con/con/pp_chart
.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/res/impr_cha
rt.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/res/pp_cha
rt.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_tim/tim/boxplo
t_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_tim/tim/p
p_chart.png (PNG copy)>] [79.99]

Package natbib Warning: Citation `schlag2020high' on page 80 undefined on input
 line 590.


Package natbib Warning: Citation `StreamMultiSection' on page 80 undefined on i
nput line 613.

) [80.100]

LaTeX Warning: Float too large for page by 4.13483pt on input line 124.

[81.101] [82.102]
Underfull \vbox (badness 3657) has occurred while \output is active [83.103])
[84.104] (./chapters/chapter2.tex
Chapter 5.

Package natbib Warning: Citation `LocMotifClusHyperGraphPartition' on page 85 u
ndefined on input line 13.


Package natbib Warning: Citation `LocMotifClusHyperGraphPartitionExtAbs' on pag
e 85 undefined on input line 13.


Package natbib Warning: Citation `LocMotifClusMaxFlows' on page 85 undefined on
 input line 13.

(./chapters/lmcvhgp/chapter.tex [85.105]

Package natbib Warning: Citation `mqipaper2004' on page 86 undefined on input l
ine 93.

[86.106]

Package natbib Warning: Citation `leskovec2009community' on page 87 undefined o
n input line 245.

[87.107 <./chapters/lmcvhgp/LocalMotifClustering.png (PNG copy)>]

Package natbib Warning: Citation `leskovec2009community' on page 88 undefined o
n input line 250.


Package natbib Warning: Citation `read1977graph' on page 88 undefined on input 
line 267.


Package natbib Warning: Citation `ortmann2014triangle' on page 88 undefined on 
input line 268.


Package natbib Warning: Citation `holme2002growing' on page 88 undefined on inp
ut line 269.


Package natbib Warning: Citation `batagelj2007short' on page 88 undefined on in
put line 269.


Package natbib Warning: Citation `prat2012shaping' on page 88 undefined on inpu
t line 269.


Package natbib Warning: Citation `kimmig2017shared' on page 88 undefined on inp
ut line 273.


Package natbib Warning: Citation `chiba1985arboricity' on page 88 undefined on 
input line 275.


Package natbib Warning: Citation `chiba1985arboricity' on page 88 undefined on 
input line 281.


Underfull \vbox (badness 10000) has occurred while \output is active [88.108]
[89.109]
Underfull \vbox (badness 10000) has occurred while \output is active [90.110 <.
/chapters/social/ModelConstruction.png (PNG copy)>] [91.111]

Package natbib Warning: Citation `benson2016higher' on page 92 undefined on inp
ut line 392.


Package natbib Warning: Citation `yin2017local' on page 92 undefined on input l
ine 392.

[92.112 <./chapters/lmcvhgp/SmallModelConstructionGraph.png (PNG copy)>]

Package natbib Warning: Citation `yin2017local' on page 93 undefined on input l
ine 411.


Package natbib Warning: Citation `benson2016higher' on page 93 undefined on inp
ut line 415.


Package natbib Warning: Citation `yin2017local' on page 93 undefined on input l
ine 420.


Underfull \vbox (badness 4120) has occurred while \output is active [93.113]

Package natbib Warning: Citation `schlag2016k' on page 94 undefined on input li
ne 454.


Package natbib Warning: Citation `kaHIPHomePage' on page 94 undefined on input 
line 455.


Package natbib Warning: Citation `gottesburen2021scalable' on page 94 undefined
 on input line 482.


Package natbib Warning: Citation `gottesburen2021scalable' on page 94 undefined
 on input line 483.


Package natbib Warning: Citation `DBLP:conf/esa/GottesburenH00S21' on page 94 u
ndefined on input line 483.

[94.114]

Package natbib Warning: Citation `labelpropagationclustering' on page 95 undefi
ned on input line 488.

) (./chapters/social/chapter.tex

Package natbib Warning: Citation `mqipaper2004' on page 95 undefined on input l
ine 141.

[95.115] [96.116 <./chapters/social/FlowLocalMotifClustering.png (PNG copy)>]
[97.117] [98.118 <./chapters/social/FlowModel.png (PNG copy)>]

Package natbib Warning: Citation `ford_fulkerson_1956' on page 99 undefined on 
input line 291.


Package natbib Warning: Citation `ford_fulkerson_1956' on page 99 undefined on 
input line 329.

[99.119]
Overfull \hbox (13.10965pt too wide) in paragraph at lines 333--342
[]\OT1/lmr/m/n/12 (-20) Now we show that the weights of the re-main-ing cut edg
es, i.e., edges from $\OML/lmm/m/it/12 B[]$ \OT1/lmr/m/n/12 (-20) to $[]$
[100.120]

Package natbib Warning: Citation `schlag2016k' on page 101 undefined on input l
ine 373.


Package natbib Warning: Citation `kaffpa' on page 101 undefined on input line 3
73.


Package natbib Warning: Citation `yin2017local' on page 101 undefined on input 
line 382.


Package natbib Warning: Citation `zhou2021high' on page 101 undefined on input 
line 383.


Package natbib Warning: Citation `zhang2019local' on page 101 undefined on inpu
t line 387.


Package natbib Warning: Citation `yin2017local' on page 101 undefined on input 
line 396.

[101.121] [102.122]

Package natbib Warning: Citation `yin2017local' on page 103 undefined on input 
line 486.

[103.123]

Package natbib Warning: Citation `zhang2019local' on page 104 undefined on inpu
t line 554.


Package natbib Warning: Citation `zhang2019local' on page 104 undefined on inpu
t line 556.

[104.124 <./chapters/social/plots/mqi_clique/res/pp_chart.png (PNG copy)>])
[105.125 <./chapters/social/plots/mqi_clique/res/double_chart.png (PNG copy)>])
[106.126] (./chapters/chapter3.tex
Chapter 6.

Package natbib Warning: Citation `HighQualityHierarchicalPM20' on page 107 unde
fined on input line 11.


Package natbib Warning: Citation `DistrMemMLevelSigGraphClustering_short' on pa
ge 107 undefined on input line 11.


Package natbib Warning: Citation `DistrMemMLevelSigGraphClustering' on page 107
 undefined on input line 11.

(./chapters/integratedProcessMappingPaper/chapter.tex [107.127]

Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
06.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
24.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
26.


Package natbib Warning: Citation `kaffpa' on page 108 undefined on input line 2
26.

[108.128 <./chapters/integratedProcessMappingPaper/MultilevelMap.png (PNG copy)
>]

Package natbib Warning: Citation `GlobalMultisection' on page 109 undefined on 
input line 259.


Package natbib Warning: Citation `schulz2017better' on page 109 undefined on in
put line 274.


Package natbib Warning: Citation `fiduccia1982lth' on page 109 undefined on inp
ut line 293.


Underfull \vbox (badness 10000) has occurred while \output is active [109.129]

Package natbib Warning: Citation `kaffpa' on page 110 undefined on input line 3
21.


Package natbib Warning: Citation `fiduccia1982lth' on page 110 undefined on inp
ut line 323.

[110.130]

Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
36.


Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
41.


Package natbib Warning: Citation `labelpropagationclustering' on page 111 undef
ined on input line 350.


Package natbib Warning: Citation `kaffpa' on page 111 undefined on input line 3
72.


Underfull \vbox (badness 6047) has occurred while \output is active [111.131]
[112.132 <./chapters/integratedProcessMappingPaper/bin_rep.png (PNG copy)>]

Package natbib Warning: Citation `schlag2016k' on page 113 undefined on input l
ine 478.

[113.133]

Package natbib Warning: Citation `kaffpa' on page 114 undefined on input line 5
33.


Package natbib Warning: Citation `kaffpa' on page 114 undefined on input line 5
34.


Package natbib Warning: Citation `schulz2017better' on page 114 undefined on in
put line 535.


Package natbib Warning: Citation `muller2013optimale' on page 114 undefined on 
input line 538.


Package natbib Warning: Citation `schulz2017better' on page 114 undefined on in
put line 538.


Package natbib Warning: Citation `Scotch' on page 114 undefined on input line 5
39.


Package natbib Warning: Citation `GlobalMultisection' on page 114 undefined on 
input line 541.


Package natbib Warning: Citation `Scotch' on page 114 undefined on input line 5
44.


Package natbib Warning: Citation `walshaw2000mpm' on page 114 undefined on inpu
t line 547.


Underfull \vbox (badness 2865) has occurred while \output is active [114.134]

Package natbib Warning: Citation `schulz2017better' on page 115 undefined on in
put line 629.

[115.135] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmr.fd) [116.136 
<./chapters/integratedProcessMappingPaper/Results/InitSol/result.png (PNG copy)
> <./chapters/integratedProcessMappingPaper/Results/InitSol/time.png (PNG copy)
>] [117.137] [118.138 <./chapters/integratedProcessMappingPaper/Results/Refinem
ent/result_eco.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Result
s/Refinement/time_eco.png (PNG copy)>]
Overfull \hbox (8.57442pt too wide) in paragraph at lines 809--822
[]\OT1/lmr/m/n/12 (-20) We now high-light the com-par-i-son of var-i-ous con-fi
g-u-ra-tions/algorithms. $[]$
[119.139 <./chapters/integratedProcessMappingPaper/Results/DistMatrix/time_stro
ng.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/result_glo
b.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/time_glob.p
ng (PNG copy)>]) (./chapters/SignedClusterEvolutionaryPaper/chapter.tex
[120.140]

Package natbib Warning: Citation `labelpropagationclustering' on page 121 undef
ined on input line 261.

[121.141]

Package natbib Warning: Citation `fiduccia1982lth' on page 122 undefined on inp
ut line 301.


Package natbib Warning: Citation `labelpropagationclustering' on page 122 undef
ined on input line 317.

[122.142]

Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
38.


Package natbib Warning: Citation `fiduccia1982lth' on page 123 undefined on inp
ut line 338.


Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
42.


Package natbib Warning: Citation `walshaw2004multilevel' on page 123 undefined 
on input line 363.


Package natbib Warning: Citation `kaffpa' on page 123 undefined on input line 3
72.


Package natbib Warning: Citation `sanders2012distributed' on page 123 undefined
 on input line 381.

[123.143 <./chapters/SignedClusterEvolutionaryPaper/MSGC_second_cycle.png (PNG 
copy)>]

Package natbib Warning: Citation `evolutionary_book' on page 124 undefined on i
nput line 400.

[124.144]

Package natbib Warning: Citation `tournament_selection' on page 125 undefined o
n input line 457.


Underfull \vbox (badness 3219) has occurred while \output is active [125.145]

Package natbib Warning: Citation `sanders2012distributed' on page 126 undefined
 on input line 504.


Package natbib Warning: Citation `randomgossip' on page 126 undefined on input 
line 506.


Underfull \vbox (badness 10000) has occurred while \output is active [126.146 <
./chapters/SignedClusterEvolutionaryPaper/pics/recombination.png (PNG copy)>]

Package natbib Warning: Citation `bailoni2019generalized' on page 127 undefined
 on input line 530.


Package natbib Warning: Citation `bailoni2019generalized' on page 127 undefined
 on input line 531.


Package natbib Warning: Citation `keuper2015efficient' on page 127 undefined on
 input line 531.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 533.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 534.


Package natbib Warning: Citation `HuaRandomWalk2020' on page 127 undefined on i
nput line 547.

[127.147]

Package natbib Warning: Citation `sanders2012distributed' on page 128 undefined
 on input line 560.

[128.148]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `tbp') on input line 639.

[129.149 <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores
/conv/all/double_chart.png (PNG copy)>])
Underfull \vbox (badness 10000) has occurred while \output is active [130.150 <
./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores/conv/soc-
sign-Slashdot090216/double_chart.png (PNG copy)> <./chapters/SignedClusterEvolu
tionaryPaper/pics/convergence_1h_16cores/conv/soc-sign-epinions/double_chart.pn
g (PNG copy)> <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16
cores/conv/wikisigned-k2/double_chart.png (PNG copy)> <./chapters/SignedCluster
EvolutionaryPaper/pics/convergence_1h_16cores/conv/slashdot-zoo/double_chart.pn
g (PNG copy)>] [131.151]) [132.152] (./chapters/discussion.tex
Chapter 7.
[133.153] [134.154]) [135.155] [136.156] (./main.bbl [137.157]
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmtt.fd) [138.158] [139.159
]
Underfull \hbox (badness 2653) in paragraph at lines 227--232
\OT1/lmr/m/it/12 (+20) ing and Fight-ing Cy-ber Ter-ror-ism (IBIGDELFT)\OT1/lmr
/m/n/12 (+20) , pages 65--70, 2018.

Underfull \hbox (badness 2318) in paragraph at lines 251--257
\OT1/lmr/m/n/12 (+20) or-ga-ni-za-tion of com-plex net-works.  \OT1/lmr/m/it/12
 (+20) Sci-ence\OT1/lmr/m/n/12 (+20) , 353(6295):163--166, 2016.
[140.160]
Underfull \hbox (badness 10000) in paragraph at lines 317--323
\OT1/lmtt/m/n/12 ac . id / id / eprint / 271 / 1 / 2014 _ Book _ SearchMethodol
ogies . pdf # page = 106$[]\OT1/lmr/m/n/12 (+20) .
[141.161] [142.162] [143.163]
Underfull \hbox (badness 1178) in paragraph at lines 508--513
[]\OT1/lmr/m/n/12 (+20) Lars Gottesb^^?uren, To-bias Heuer, Pe-ter Sanders, and
 Se-bas-tian Schlag.
[144.164] [145.165]
Underfull \hbox (badness 2582) in paragraph at lines 624--629
\OT1/lmr/m/n/12 (+20) doi:[]10.1145/3038912.3052653[].  URL []$\OT1/lmtt/m/n/12
 https : / / doi . org / 10 . 1145 / 3038912 .
[146.166] [147.167]
Underfull \hbox (badness 1521) in paragraph at lines 796--803
[]\OT1/lmr/m/n/12 (+20) ataly^^?urek.  Multi-jagged: A scal-able par-al-lel spa
-tial par-ti-tion-ing al-

Underfull \hbox (badness 1275) in paragraph at lines 796--803
\OT1/lmr/m/n/12 (+20) go-rithm.  \OT1/lmr/m/it/12 (+20) IEEE Trans. Par-al-lel 
Dis-tributed Syst.\OT1/lmr/m/n/12 (+20) , 27(3):803--817, 2016.
[148.168] [149.169] [150.170] [151.171] [152.172]
Underfull \hbox (badness 2057) in paragraph at lines 1147--1153
[]\OT1/lmr/m/n/12 (+20) Adil Chhabra, Marcelo Fon-seca Faraj, and Chris-tian Sc
hulz.  Lo-cal

Underfull \hbox (badness 1527) in paragraph at lines 1147--1153
\OT1/lmr/m/n/12 (+20) mo-tif clus-ter-ing via (hy-per)graph par-ti-tion-ing.  I
n \OT1/lmr/m/it/12 (+20) 2023 Proc. of the
[153.173] [154.174]
Underfull \hbox (badness 10000) in paragraph at lines 1292--1297
[]\OT1/lmr/m/n/12 (+20) Chris Wal-shaw.  Mul-ti-level re-fine-ment for com-bi-n
a-to-rial op-ti-

Underfull \hbox (badness 10000) in paragraph at lines 1292--1297
\OT1/lmr/m/n/12 (+20) mi-sa-tion prob-lems.  \OT1/lmr/m/it/12 (+20) Ann. Oper. 
Res.\OT1/lmr/m/n/12 (+20) , 131(1-4):325--372, 2004.

Underfull \hbox (badness 6125) in paragraph at lines 1292--1297
\OT1/lmr/m/n/12 (+20) doi:[]10.1023/B:ANOR.0000039525.80601.15[].  URL []$\OT1/
lmtt/m/n/12 https : / / doi . org / 10 .
[155.175]) [156.176] (./chapters/curriculum.tex [157.177] [158.178])
(./chapters/allpublications.tex [159.179] [160.180] [161.181])

Package natbib Warning: There were undefined citations.

(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-utf8.def)
(./main.aux (./chapters/abstracts.aux) (./chapters/acknowledgements.aux)
(./chapters/publications.aux) (./chapters/introduction.aux)
(./chapters/preliminaries.aux) (./chapters/related_work.aux)
(./chapters/chapter1.aux) (./chapters/chapter2.aux) (./chapters/chapter3.aux)
(./chapters/discussion.aux)

Package natbib Warning: Citation(s) may have changed.
(natbib)                Rerun to get citations correct.

(./chapters/curriculum.aux) (./chapters/allpublications.aux))

LaTeX Warning: There were multiply-defined labels.


Package rerunfilecheck Warning: File `main.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.

 )
(see the transcript file for additional information)
pdfTeX warning (dest): name{section*.120} has been referenced but does not exis
t, replaced by a fixed one

{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-rmtt.enc}{/usr/local/
texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-rm.enc}{/usr/local/texlive/2022/t
exmf-dist/fonts/enc/dvips/lm/lm-rmsc.enc}{/usr/local/texlive/2022/texmf-dist/fo
nts/enc/dvips/lm/lm-mathit.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dv
ips/lm/lm-mathsy.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-
mathex.enc}</usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmbx10.pfb
></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmbx12.pfb></usr/loc
al/texlive/2022/texmf-dist/fonts/type1/public/lm/lmbx8.pfb></usr/local/texlive/
2022/texmf-dist/fonts/type1/public/lm/lmcsc10.pfb></usr/local/texlive/2022/texm
f-dist/fonts/type1/public/lm/lmex10.pfb></usr/local/texlive/2022/texmf-dist/fon
ts/type1/public/lm/lmmi10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/p
ublic/lm/lmmi12.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/l
mmi6.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi8.pfb></
usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr10.pfb></usr/local/t
exlive/2022/texmf-dist/fonts/type1/public/lm/lmr12.pfb></usr/local/texlive/2022
/texmf-dist/fonts/type1/public/lm/lmr17.pfb></usr/local/texlive/2022/texmf-dist
/fonts/type1/public/lm/lmr6.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1
/public/lm/lmr7.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/l
mr8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmri12.pfb></
usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmss10.pfb></usr/local/
texlive/2022/texmf-dist/fonts/type1/public/lm/lmss12.pfb></usr/local/texlive/20
22/texmf-dist/fonts/type1/public/lm/lmss8.pfb></usr/local/texlive/2022/texmf-di
st/fonts/type1/public/lm/lmsy10.pfb></usr/local/texlive/2022/texmf-dist/fonts/t
ype1/public/lm/lmsy6.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public
/lm/lmsy8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmtt12.
pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/amsfonts/symbols/msb
m10.pfb>
Output written on main.pdf (181 pages, 9714547 bytes).
SyncTeX written on main.synctex.gz.
Transcript written on main.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.24 (TeX Live 2022) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2021-11-15> patch level 1
L3 programming layer <2022-02-24> (./hdphdthesis.cls
Document Class: hdphdthesis 08 Jan 2022 Heidelberg University Dr. rer. nat. The
sis class
(/usr/local/texlive/2022/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/book.cls
Document Class: book 2021/10/04 v1.4n Standard LaTeX document class
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/bk12.clo))
(/usr/local/texlive/2022/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifvtex.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/iftex.sty)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.te
x
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-common-li
sts.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def
) (/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeysfiltered.c
ode.tex))) (/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex
)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.
tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigo
nometric.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.rando
m.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.compa
rison.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integ
erarithmetics.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex)
))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/sttools/stfloats.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/cite/cite.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/caption3.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjustbox.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/adjcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/trimclip.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/collectbox/collectbox.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/adjustbox/tc-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifoddpage/ifoddpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/varwidth/varwidth.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/emptypage/emptypage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/array.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/afterpage.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/lmodern.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/float/float.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/placeins/placeins.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/preprint/balance.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/inputenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/url/url.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithms/algorithm.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/ifthen.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algpseudocode.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/algorithmicx/algorithmicx.sty
Document Style algorithmicx 1.2 - a greatly improved `algorithmic' style
)
Document Style - pseudocode environments for use with the `algorithmicx' style
) (/usr/local/texlive/2022/texmf-dist/tex/latex/numprint/numprint.sty
No configuration file `numprint.cfg' found.)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amscls/amsthm.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvsetkeys/kvsetkeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pdfescape/pdfescape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/kvoptions/kvoptions.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/local/texlive/2022/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty

(/usr/local/texlive/2022/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty
))) (/usr/local/texlive/2022/texmf-dist/tex/latex/tools/xspace.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/wrapfig/wrapfig.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics-cfg/color.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.d
ef
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-p
df.def)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconst
ruct.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage
.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicst
ate.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransform
ations.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.c
ode.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathproce
ssing.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.
code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.co
de.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretranspare
ncy.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.
code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.
tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.
tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-0-65.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version
-1-18.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.cod
e.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothan
dlers.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.cod
e.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarytopaths.code.tex)))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarypositioning.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/calc.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/threeparttable/threeparttable.sty
) (/usr/local/texlive/2022/texmf-dist/tex/latex/hvfloat/hvfloat.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/picture/picture.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))
(/usr/local/texlive/2022/texmf-dist/tex/latex/multido/multido.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/multido/multido.tex
 v1.42, 2010/05/14 <tvz>)))
(/usr/local/texlive/2022/texmf-dist/tex/latex/natbib/natbib.sty

Package natbib Warning: The `cite' package should not be used
(natbib)                with natbib. Use option `sort' instead.

) (/usr/local/texlive/2022/texmf-dist/tex/latex/doi/doi.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/multicol.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibraryshapes.arrows.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibrary
shapes.arrows.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarychains.code.tex)
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.pathreplacing.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/frontendlayer/tikz/librarie
s/tikzlibrarydecorations.code.tex
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/modules/pgfmoduledecoration
s.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/generic/pgf/libraries/decorations/pgfli
brarydecorations.pathreplacing.code.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/framed/framed.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/amsfonts.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/xifthen/xifthen.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/local/texlive/2022/texmf-dist/tex/latex/tools/verbatim.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/local/texlive/2022/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/local/texlive/2022/texmf-dist/tex/latex/doclicense/doclicense-english.ldf
)) (/usr/local/texlive/2022/texmf-dist/tex/latex/ccicons/ccicons.sty)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.def)
(/usr/local/texlive/2022/texmf-dist/tex/latex/csquotes/csquotes.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmr.fd)

LaTeX Warning: Unused global option(s):
    [mathcomp,marginleft,marginright,margintop,marginbottom,bindingoffset].

(./main.aux (./chapters/abstracts.aux) (./chapters/acknowledgements.aux)
(./chapters/publications.aux) (./chapters/introduction.aux)
(./chapters/preliminaries.aux) (./chapters/related_work.aux)
(./chapters/chapter1.aux) (./chapters/chapter2.aux

LaTeX Warning: Label `sec:lmcvhgp_Local Motif Clustering via (Hyper)Graph Parti
tioning' multiply defined.

) (./chapters/chapter3.aux

LaTeX Warning: Label `subsec:Parameter Study' multiply defined.


LaTeX Warning: Label `sec:sgc_Multilevel Signed Graph Clustering' multiply defi
ned.

) (./chapters/discussion.aux) (./chapters/curriculum.aux)
(./chapters/allpublications.aux))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/local/texlive/2022/texmf-dist/tex/latex/caption/ltcaption.sty)
(/usr/local/texlive/2022/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/local/texlive/2022/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
(/usr/local/texlive/2022/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/local/texlive/2022/texmf-dist/tex/latex/refcount/refcount.sty)
(/usr/local/texlive/2022/texmf-dist/tex/generic/gettitlestring/gettitlestring.s
ty)) (./main.out) (./main.out)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-cmr.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omllmm.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmsy.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omxlmex.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/local/texlive/2022/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/local/texlive/2022/texmf-dist/tex/latex/microtype/mt-msb.cfg) [1.1{/usr/l
ocal/texlive/2022/texmf-var/fonts/map/pdftex/updmap/pdftex.map}] [2.2] [3.3]
[4.4] (./chapters/abstracts.tex [5.5] [6.6]
Underfull \hbox (badness 5696) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Dis-ser-ta-tion be-fasst sich mit der Un-ter-suchung ver-
schiedener Arten von

Underfull \hbox (badness 6708) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) Multi-Level-Algorithmen. Im Bere-ich der Streaming-Algori
thmen leis-ten

Underfull \hbox (badness 10000) in paragraph at lines 15--25
\OT1/lmr/m/n/12 (+20) wir Beitr^^?age mit hochef-fizien-ten und ef-fek-tiven Al
-go-rith-men f^^?ur die
[7.7]) (./chapters/acknowledgements.tex [8.8]
Underfull \vbox (badness 1533) has occurred while \output is active [9.9]
Underfull \vbox (badness 1515) has occurred while \output is active [10.10]
[11.11]) (./chapters/publications.tex [12.12]
Underfull \hbox (badness 10000) in paragraph at lines 2--3

[13.13] [14.14] [15.15]) [16.16] (./main.toc [17.17] [18.18]) [19.19] [20.20]
(./chapters/introduction.tex
Chapter 1.
[1.21]
Underfull \vbox (badness 10000) has occurred while \output is active [2.22]
[3.23] [4.24] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmss.fd)
[5.25] [6.26]) [7.27] (./chapters/preliminaries.tex [8.28]
Chapter 2.
[9.29] [10.30] [11.31] [12.32]
Underfull \vbox (badness 10000) has occurred while \output is active [13.33]
[14.34 <./chapters/social/HyperEdgeExpansions.png (PNG copy)>] [15.35 <./chapte
rs/heistream/pics/MGP.png (PNG copy)> <./chapters/SignedClusterEvolutionaryPape
r/pics/cluster_contraction.png (PNG copy)>]
Underfull \vbox (badness 10000) has occurred while \output is active [16.36 <./
chapters/SignedClusterEvolutionaryPaper/pics/LP_illustration.png (PNG copy)>]
[17.37 <./chapters/more_recent_partitioning_survey/img/streaming/streaming.png 
(PNG copy)>] [18.38]
Underfull \vbox (badness 10000) has occurred while \output is active [19.39]
[20.40] [21.41 <./chapters/social/plots/mqi_clique/tim/pp_chart.png (PNG copy)>
]) [22.42] (./chapters/related_work.tex
Chapter 3.
[23.43] [24.44] [25.45] [26.46] [27.47]
Underfull \vbox (badness 3657) has occurred while \output is active [28.48]
[29.49]
Underfull \vbox (badness 3590) has occurred while \output is active [30.50]
Underfull \vbox (badness 1515) has occurred while \output is active [31.51]
Underfull \vbox (badness 10000) has occurred while \output is active [32.52]
[33.53]
Underfull \vbox (badness 10000) has occurred while \output is active [34.54]
[35.55]) [36.56] (./chapters/chapter1.tex
Chapter 4.
(./chapters/heistream/chapter.tex
Underfull \vbox (badness 10000) has occurred while \output is active [37.57]
[38.58]
Underfull \vbox (badness 10000) has occurred while \output is active [39.59 <./
chapters/heistream/MultilevelBufferedStreamGP.png (PNG copy)>] [40.60] [41.61]
[42.62]
Underfull \vbox (badness 10000) has occurred while \output is active [43.63]
[44.64] [45.65] [46.66] [47.67 <./chapters/heistream/Images/repetitions_label_p
rop/res_rep_label.png (PNG copy)> <./chapters/heistream/Images/tim_TIMErep_labe
l/tim_TIMErep_label.png (PNG copy)> <./chapters/heistream/Images/StopRule/res_S
topRule.png (PNG copy)> <./chapters/heistream/Images/restream/res_restream.png 
(PNG copy)> <./chapters/heistream/Images/batch_noFennel/res_batch_noFennel.png 
(PNG copy)> <./chapters/heistream/Images/tim_TIMEbatch_noFennel/tim_TIMEbatch_n
oFennel.png (PNG copy)>]
Underfull \vbox (badness 1348) has occurred while \output is active [48.68 <./c
hapters/heistream/Images/ghost/res_ghost.png (PNG copy)> <./chapters/heistream/
Images/tim_TIMEghost/tim_TIMEghost.png (PNG copy)>]
Overfull \hbox (11.6059pt too wide) in paragraph at lines 665--701
 [][] 
[49.69 <./chapters/heistream/Images/MultiLDG/comparison_MultiLDG_vertical/Multi
LDGFullBuffer.png (PNG copy)>] [50.70] [51.71 <./chapters/heistream/Images/res_
stateOfTheArtPlots/res_stateOfTheArtPlots.png (PNG copy)> <./chapters/heistream
/Images/tim_stateOfTheArtPlots/tim_stateOfTheArtPlots.png (PNG copy)> <./chapte
rs/heistream/Images/res_stateOfTheArtPlots/pp_res_stateOfTheArtPlots.png (PNG c
opy)> <./chapters/heistream/Images/tim_stateOfTheArtPlots/pp_tim_stateOfTheArtP
lots.png (PNG copy)>]
Underfull \vbox (badness 5939) has occurred while \output is active [52.72 <./c
hapters/heistream/Images/res_restreamStateOfTheArtPlots/pp_res_restreamStateOfT
heArtPlots.png (PNG copy)>] [53.73] [54.74 <./chapters/heistream/Visualization.
png (PNG copy)>]
Overfull \hbox (0.9859pt too wide) in paragraph at lines 867--940
 [][] 

LaTeX Warning: Float too large for page by 23.98486pt on input line 942.

[55.75] [56.76]) (./chapters/recmultisec/chapter.tex [57.77]
Underfull \vbox (badness 2012) has occurred while \output is active [58.78]
[59.79 <./chapters/recmultisec/Multi-Section.png (PNG copy)>] [60.80] [61.81]
[62.82]
Underfull \vbox (badness 10000) has occurred while \output is active [63.83]
[64.84]
Overfull \hbox (0.77881pt too wide) in paragraph at lines 798--799
\OT1/lmr/m/n/12 (-20) In this sec-tion, we show ex-per-i-ments in which we com-
pare $[]$
[65.85] [66.86 <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/chart
.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartMap/res/pp_
chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/re
s/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoftheartPar/
tim/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateofthear
tPar/GP/pp_chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/stateoft
heartPar/tim/chart.png (PNG copy)>] [67.87 <./chapters/recmultisec/Images/tunin
g/parallelSpeedups/speedup/soc-orkut-dir/chart.png (PNG copy)> <./chapters/recm
ultisec/Images/tuning/parallelSpeedups/times/soc-orkut-dir/chart.png (PNG copy)
> <./chapters/recmultisec/Images/tuning/parallelSpeedups/speedup/HV15R/chart.pn
g (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/times/HV15
R/chart.png (PNG copy)> <./chapters/recmultisec/Images/tuning/parallelSpeedups/
speedup/soc-LiveJournal1/chart.png (PNG copy)> <./chapters/recmultisec/Images/t
uning/parallelSpeedups/times/soc-LiveJournal1/chart.png (PNG copy)>] [68.88])
(./chapters/freight/chapter.tex [69.89] [70.90]
Overfull \hbox (10.08015pt too wide) in paragraph at lines 181--185
\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m/it/12 V[]\OT1/lmr/m/n/12 (-
20) )[]$, where the weight $\OML/lmm/m/it/12 c\OT1/lmr/m/n/12 (-20) (\OML/lmm/m
/it/12 v\OT1/lmr/m/n/12 (-20) )$ of $\OML/lmm/m/it/12 v$ \OT1/lmr/m/n/12 (-20) 
is []. 
[71.91 <./chapters/freight/streaming.png (PNG copy)>] [72.92]
Underfull \vbox (badness 1694) has occurred while \output is active [73.93 <./c
hapters/freight/DecomposeEqFREIGHT.png (PNG copy)>]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `htbp') on input line 305.

[74.94 <./chapters/freight/SortingArrays.png (PNG copy)>] [75.95]
Overfull \hbox (0.97314pt too wide) in paragraph at lines 411--420
[]\OT1/lmr/m/n/12 (-20) We run $[]$, $[]$ [[]] and its im-proved ver-sions pro-
posed in  [[]]: $[]$,
[76.96] [77.97] [78.98 <./chapters/freight/Images/allhypergraphs_all_con/con/im
pr_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_con/con/
pp_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/res/
impr_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_cut/re
s/pp_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_tim/ti
m/boxplot_chart.png (PNG copy)> <./chapters/freight/Images/allhypergraphs_all_t
im/tim/pp_chart.png (PNG copy)>] [79.99]) [80.100]

LaTeX Warning: Float too large for page by 4.13483pt on input line 124.

[81.101] [82.102]
Underfull \vbox (badness 3657) has occurred while \output is active [83.103])
[84.104] (./chapters/chapter2.tex
Chapter 5.
(./chapters/lmcvhgp/chapter.tex [85.105] [86.106] [87.107 <./chapters/lmcvhgp/L
ocalMotifClustering.png (PNG copy)>]
Underfull \vbox (badness 10000) has occurred while \output is active [88.108]
[89.109]
Underfull \vbox (badness 10000) has occurred while \output is active [90.110 <.
/chapters/social/ModelConstruction.png (PNG copy)>] [91.111] [92.112 <./chapter
s/lmcvhgp/SmallModelConstructionGraph.png (PNG copy)>]
Underfull \vbox (badness 4120) has occurred while \output is active [93.113]
[94.114]) (./chapters/social/chapter.tex [95.115] [96.116 <./chapters/social/Fl
owLocalMotifClustering.png (PNG copy)>] [97.117] [98.118 <./chapters/social/Flo
wModel.png (PNG copy)>] [99.119]
Overfull \hbox (13.10965pt too wide) in paragraph at lines 333--342
[]\OT1/lmr/m/n/12 (-20) Now we show that the weights of the re-main-ing cut edg
es, i.e., edges from $\OML/lmm/m/it/12 B[]$ \OT1/lmr/m/n/12 (-20) to $[]$
[100.120] [101.121] [102.122] [103.123] [104.124 <./chapters/social/plots/mqi_c
lique/res/pp_chart.png (PNG copy)>]) [105.125 <./chapters/social/plots/mqi_cliq
ue/res/double_chart.png (PNG copy)>]) [106.126] (./chapters/chapter3.tex
Chapter 6.
(./chapters/integratedProcessMappingPaper/chapter.tex [107.127] [108.128 <./cha
pters/integratedProcessMappingPaper/MultilevelMap.png (PNG copy)>]
Underfull \vbox (badness 10000) has occurred while \output is active [109.129]
[110.130]
Underfull \vbox (badness 6047) has occurred while \output is active [111.131]
[112.132 <./chapters/integratedProcessMappingPaper/bin_rep.png (PNG copy)>]
[113.133]
Underfull \vbox (badness 2865) has occurred while \output is active [114.134]
[115.135] (/usr/local/texlive/2022/texmf-dist/tex/latex/lm/omslmr.fd) [116.136 
<./chapters/integratedProcessMappingPaper/Results/InitSol/result.png (PNG copy)
> <./chapters/integratedProcessMappingPaper/Results/InitSol/time.png (PNG copy)
>] [117.137] [118.138 <./chapters/integratedProcessMappingPaper/Results/Refinem
ent/result_eco.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Result
s/Refinement/time_eco.png (PNG copy)>]
Overfull \hbox (8.57442pt too wide) in paragraph at lines 809--822
[]\OT1/lmr/m/n/12 (-20) We now high-light the com-par-i-son of var-i-ous con-fi
g-u-ra-tions/algorithms. $[]$
[119.139 <./chapters/integratedProcessMappingPaper/Results/DistMatrix/time_stro
ng.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/result_glo
b.png (PNG copy)> <./chapters/integratedProcessMappingPaper/Results/time_glob.p
ng (PNG copy)>]) (./chapters/SignedClusterEvolutionaryPaper/chapter.tex
[120.140] [121.141] [122.142] [123.143 <./chapters/SignedClusterEvolutionaryPap
er/MSGC_second_cycle.png (PNG copy)>] [124.144]
Underfull \vbox (badness 3219) has occurred while \output is active [125.145]
Underfull \vbox (badness 10000) has occurred while \output is active [126.146 <
./chapters/SignedClusterEvolutionaryPaper/pics/recombination.png (PNG copy)>]
[127.147] [128.148]

LaTeX Warning: No positions in optional float specifier.
               Default added (so using `tbp') on input line 639.

[129.149 <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores
/conv/all/double_chart.png (PNG copy)>])
Underfull \vbox (badness 10000) has occurred while \output is active [130.150 <
./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16cores/conv/soc-
sign-Slashdot090216/double_chart.png (PNG copy)> <./chapters/SignedClusterEvolu
tionaryPaper/pics/convergence_1h_16cores/conv/soc-sign-epinions/double_chart.pn
g (PNG copy)> <./chapters/SignedClusterEvolutionaryPaper/pics/convergence_1h_16
cores/conv/wikisigned-k2/double_chart.png (PNG copy)> <./chapters/SignedCluster
EvolutionaryPaper/pics/convergence_1h_16cores/conv/slashdot-zoo/double_chart.pn
g (PNG copy)>] [131.151]) [132.152] (./chapters/discussion.tex
Chapter 7.
[133.153] [134.154]) [135.155] [136.156] (./main.bbl [137.157]
(/usr/local/texlive/2022/texmf-dist/tex/latex/lm/ot1lmtt.fd) [138.158] [139.159
]
Underfull \hbox (badness 2653) in paragraph at lines 227--232
\OT1/lmr/m/it/12 (+20) ing and Fight-ing Cy-ber Ter-ror-ism (IBIGDELFT)\OT1/lmr
/m/n/12 (+20) , pages 65--70, 2018.

Underfull \hbox (badness 2318) in paragraph at lines 251--257
\OT1/lmr/m/n/12 (+20) or-ga-ni-za-tion of com-plex net-works.  \OT1/lmr/m/it/12
 (+20) Sci-ence\OT1/lmr/m/n/12 (+20) , 353(6295):163--166, 2016.
[140.160]
Underfull \hbox (badness 10000) in paragraph at lines 317--323
\OT1/lmtt/m/n/12 ac . id / id / eprint / 271 / 1 / 2014 _ Book _ SearchMethodol
ogies . pdf # page = 106$[]\OT1/lmr/m/n/12 (+20) .
[141.161] [142.162] [143.163]
Underfull \hbox (badness 1178) in paragraph at lines 508--513
[]\OT1/lmr/m/n/12 (+20) Lars Gottesb^^?uren, To-bias Heuer, Pe-ter Sanders, and
 Se-bas-tian Schlag.
[144.164] [145.165]
Underfull \hbox (badness 2582) in paragraph at lines 624--629
\OT1/lmr/m/n/12 (+20) doi:[]10.1145/3038912.3052653[].  URL []$\OT1/lmtt/m/n/12
 https : / / doi . org / 10 . 1145 / 3038912 .
[146.166] [147.167]
Underfull \hbox (badness 1521) in paragraph at lines 796--803
[]\OT1/lmr/m/n/12 (+20) ataly^^?urek.  Multi-jagged: A scal-able par-al-lel spa
-tial par-ti-tion-ing al-

Underfull \hbox (badness 1275) in paragraph at lines 796--803
\OT1/lmr/m/n/12 (+20) go-rithm.  \OT1/lmr/m/it/12 (+20) IEEE Trans. Par-al-lel 
Dis-tributed Syst.\OT1/lmr/m/n/12 (+20) , 27(3):803--817, 2016.
[148.168] [149.169] [150.170] [151.171] [152.172]
Underfull \hbox (badness 2057) in paragraph at lines 1147--1153
[]\OT1/lmr/m/n/12 (+20) Adil Chhabra, Marcelo Fon-seca Faraj, and Chris-tian Sc
hulz.  Lo-cal

Underfull \hbox (badness 1527) in paragraph at lines 1147--1153
\OT1/lmr/m/n/12 (+20) mo-tif clus-ter-ing via (hy-per)graph par-ti-tion-ing.  I
n \OT1/lmr/m/it/12 (+20) 2023 Proc. of the
[153.173] [154.174]
Underfull \hbox (badness 10000) in paragraph at lines 1292--1297
[]\OT1/lmr/m/n/12 (+20) Chris Wal-shaw.  Mul-ti-level re-fine-ment for com-bi-n
a-to-rial op-ti-

Underfull \hbox (badness 10000) in paragraph at lines 1292--1297
\OT1/lmr/m/n/12 (+20) mi-sa-tion prob-lems.  \OT1/lmr/m/it/12 (+20) Ann. Oper. 
Res.\OT1/lmr/m/n/12 (+20) , 131(1-4):325--372, 2004.

Underfull \hbox (badness 6125) in paragraph at lines 1292--1297
\OT1/lmr/m/n/12 (+20) doi:[]10.1023/B:ANOR.0000039525.80601.15[].  URL []$\OT1/
lmtt/m/n/12 https : / / doi . org / 10 .
[155.175]) [156.176] (./chapters/curriculum.tex [157.177] [158.178])
(./chapters/allpublications.tex [159.179] [160.180] [161.181])
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/local/texlive/2022/texmf-dist/tex/generic/stringenc/se-utf8.def)
(./main.aux (./chapters/abstracts.aux) (./chapters/acknowledgements.aux)
(./chapters/publications.aux) (./chapters/introduction.aux)
(./chapters/preliminaries.aux) (./chapters/related_work.aux)
(./chapters/chapter1.aux) (./chapters/chapter2.aux) (./chapters/chapter3.aux)
(./chapters/discussion.aux) (./chapters/curriculum.aux)
(./chapters/allpublications.aux))

LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){/usr/local/texlive/2022/te
xmf-dist/fonts/enc/dvips/lm/lm-rmtt.enc}{/usr/local/texlive/2022/texmf-dist/fon
ts/enc/dvips/lm/lm-rm.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/l
m/lm-rmsc.enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathit.
enc}{/usr/local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathsy.enc}{/usr/
local/texlive/2022/texmf-dist/fonts/enc/dvips/lm/lm-mathex.enc}</usr/local/texl
ive/2022/texmf-dist/fonts/type1/public/lm/lmbx10.pfb></usr/local/texlive/2022/t
exmf-dist/fonts/type1/public/lm/lmbx12.pfb></usr/local/texlive/2022/texmf-dist/
fonts/type1/public/lm/lmbx8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1
/public/lm/lmcsc10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/l
m/lmex10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi10.p
fb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi12.pfb></usr/l
ocal/texlive/2022/texmf-dist/fonts/type1/public/lm/lmmi6.pfb></usr/local/texliv
e/2022/texmf-dist/fonts/type1/public/lm/lmmi8.pfb></usr/local/texlive/2022/texm
f-dist/fonts/type1/public/lm/lmr10.pfb></usr/local/texlive/2022/texmf-dist/font
s/type1/public/lm/lmr12.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/pub
lic/lm/lmr17.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr6
.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr7.pfb></usr/l
ocal/texlive/2022/texmf-dist/fonts/type1/public/lm/lmr8.pfb></usr/local/texlive
/2022/texmf-dist/fonts/type1/public/lm/lmri12.pfb></usr/local/texlive/2022/texm
f-dist/fonts/type1/public/lm/lmss10.pfb></usr/local/texlive/2022/texmf-dist/fon
ts/type1/public/lm/lmss12.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/p
ublic/lm/lmss8.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lm
sy10.pfb></usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmsy6.pfb></
usr/local/texlive/2022/texmf-dist/fonts/type1/public/lm/lmsy8.pfb></usr/local/t
exlive/2022/texmf-dist/fonts/type1/public/lm/lmtt12.pfb></usr/local/texlive/202
2/texmf-dist/fonts/type1/public/amsfonts/symbols/msbm10.pfb>
Output written on main.pdf (181 pages, 9727824 bytes).
SyncTeX written on main.synctex.gz.
Transcript written on main.log.

